Tight Certificates of Adversarial Robustness for Randomly Smoothed Classifiers

Strong theoretical guarantees of robustness can be given for ensembles of classifiers generated by input randomization. Specifically, an $\ell_2$ bounded adversary cannot alter the ensemble prediction generated by an additive isotropic Gaussian noise, where the radius for the adversary depends on both the variance of the distribution as well as the ensemble margin at the point of interest. We build on and considerably expand this work across broad classes of distributions. In particular, we offer adversarial robustness guarantees and associated algorithms for the discrete case where the adversary is $\ell_0$ bounded. Moreover, we exemplify how the guarantees can be tightened with specific assumptions about the function class of the classifier such as a decision tree. We empirically illustrate these results with and without functional restrictions across image and molecule datasets.

==> backup.tex <==

\clearpage



\subsection{Inference (computing the integral)}

% \header{Deep Networks} Use techniques from Zico's paper...


\header{Decision Tree} A decision tree model $f_\theta$ partitions the space $\sR^d$ into $l$ different regions $\gW_1,\dots,\gW_l$ with axis-parallel cuts. Each region is associated with a constant output $c_i \in \gC, \forall i \in [l]$. We can decompose the probability as
\begin{align}
    \Pr (f_\theta(\rand(\vx)) = c) = \sum_{j=1}^l \Pr (\rand(\vx) \in \gW_j) \one\{ c_j = c \},
\end{align}
where all the $\Pr (\rand(\vx) \in \gW_j)$ can be computed in a depth-first search. For example, we may maintain a stack that stores all the historical splits $\one\{ \vz_i > \tau \}$, where $\Pr (\rand(\vx) \in \gW_j)$ is simply the product of the likelihood of the historical splits. 

\textred{Only true in the binary case, in the $\{K\}^d$ case, we have to futher consider when multiple splits share the same coordinate, although still feasible.}

\textred{This trick is not restricted to our perturbation, but also Gaussian perturbation in $\sR^d$.}

\subsection{Learning}

% \header{Deep Networks} To train the randomized classifier, it is essential to include the randomized signal into the training procedure. Prior works have proposed to optimize
% \begin{align}
%     \min_\theta \hat \sE_{(\vx, y)} \sE_{\vz = \rand(\vx)} \log \Pr(f_\theta (\vz) = y).
% \end{align}
% However, we argue that the cross-entropy loss is not ideal since it pushes the probability value of $\Pr(f_\theta (\vz) = y)$ strictly towards $1$. In practice, as long as the probability value $\Pr(f_\theta (\vz) = y) > \Pr(f_\theta (\vz) = y'), \forall y' \neq y$ achieved, we can always map $f$ to a deterministic model that outputs the class with maximal response. As a result, we instead consider the unnormalized model $f_\theta: \sR^d \to \sR^{|\gC|}$ (removing the soft-max), and minimize the loss
% \begin{align}
%     \min_\theta \hat \sE_{(\vx, y)} \sE_{\vz = \rand(\vx)} \max\{0, \lambda - f_\theta (\vz)_y + \max_{y' \neq y} f_\theta (\vz)_{y'}\}.
% \end{align}

\header{Decision Tree}
When training the decision tree, 
for every tree node, we will drop a random subset of the available features to avoid overfitting. 


Method 1: Probably just sample a bunch of points and minimize gini-index.

Method 2: 

(1) branching criterion: weighted gini-index.

\begin{align}
    \min_{\tau, d} (\sum_{i=1}^n w_{i, d, \geq \tau}) \bigg[ 1 - \sum_{y=0}^1 (\frac{\sum_{i=1}^n w_{i, d, \geq \tau} \one\{y_i = y\}}{\sum_{i=1}^n w_{i, d, \geq \tau}})^2\bigg] + (\sum_{i=1}^n w_{i, d, < \tau}) \bigg[ 1 - \sum_{y=0}^1 (\frac{\sum_{i=1}^n w_{i, d, < \tau} \one\{y_i = y\}}{\sum_{i=1}^n w_{i, d, < \tau}})^2\bigg]
\end{align}

% (2) the constant output (for $v$ leaf nodes):

% \begin{align}
%   \max_\theta \sum_{i=1}^{n_1} \sum_{j=1}^{n_0} \one\{f_\theta(\vx^1_i) > f_\theta(\vx^0_i)\} 
%   \geq \max_C \sum_{i=1}^{n_1} \sum_{j=1}^{n_0} \sum_{k=1}^v w_{\vx^1_i, k} C_k - w_{\vx^0_j, k} C_k, s.t. 1 \geq C_k \geq 0,
% \end{align}
% which can be solved by a linear program.




\subsection{Random Forest}

For random forest, we can run certify for each individual tree, and take the median as the certificate for the entire random forest. 

==> certificates.tex <==
\section{Robustness Certificates of Randomly Smoothed Classifiers}
\label{sec:certificates}

Given an input space $\gX \subseteq \sR^d$, a random perturbation $\rand$ assigns a probability mass/density $\Pr(\rand(\vx) = \vz)$ for each perturbed outcome $\vz \in \gX$; 
we associate the perturbation with a measurable classifier $f$, and consider the randomly smoothed classifier $f(\rand(\vx))$, where the probability for outputting a class $y \in \gY$ is denoted as $\Pr(f(\phi(\vx))=y)$. Note that $f$ can also be a random function. 
Under this setting, we first develop tight robustness guarantees of the probability $\Pr(f(\phi(\vx))=y)$ with applications to robustness in accuracy and area under the ROC curve (AUC) in the next sections, exemplify the framework in \xref{sec:examples}, and illustrate how the guarantees can be refined with further assumption in \xref{sec:refinement}. 

\subsection{Point-wise Robustness Certificates}

Given a classifier $f$ smoothed by perturbation $\rand$, we abbreviate the probability score $\Pr(f(\rand(\vx)) = c)$ for an input $\vx$ and label $c$ as $p$, whenever $f, \rand, \vx$ and $c$ is clear from the context. 
We first identify a tight lower bound on the probability score $\Pr(f(\rand(\bar \vx)) = c)$ for another (neighboring) point $\bar \vx \in \gX$.

Here we denote the set of measurable functions with respect to $\rand$ as $\gF$. If we assume nothing but measurability of $f$, the tight bound can be found by the minimization problem:
\begin{equation}
\min_{\bar{f} \in \gF: \Pr(\bar{f}(\rand(\vx)) = c) = p}
    \Pr(\bar{f}(\rand(\bar{\vx})) = c) \triangleq \rho_{\vx, \bar \vx,c}(p).
\label{eqn:target}    
\end{equation}

Intuitively, we can cast the optimization problem~(\ref{eqn:target}) as an assignment problem that initialize $\bar f(\vz) \neq c, \forall \vz \in \gX$, and then assign $\bar f(\vz) = c$ for some $\vz \in \gX$ until the constraint is met. Then a greedy strategy that assigns $\bar f(\vz) = c$ in the order of decreasing likelihood ratio $\Pr(\rand(\vx) = \vz) / \Pr(\rand(\bar \vx) = \vz)$ will achieve the minimum since the objective and the constraint can be rewritten as the measure over the input space where $\bar f(\vz) = c$ with respect to the corresponding perturbations. 

However, the above argument assumes that $\gX$ is countable and the optimal $\bar f$ is deterministic. 
Below we formally follow the idea to solve Eq.~(\ref{eqn:target}) without the assumptions.
For each point $\vz \in \gX$, we define the likelihood ratio $\eta_{\vx, \bar \vx}(\vz)\triangleq \Pr(\rand(\vx) = \vz) / \Pr(\rand(\bar \vx) = \vz)$\footnote{If $\Pr(\rand(\bar \vx) = \vz) = \Pr(\rand(\vx) = \vz) = 0$, $\eta_{\vx, \bar \vx}(\vz)$ is defined arbitrarily in $[0, \infty)$.}.
If we can partition $\gX$ into $n$ regions $\gL_1 \dots \gL_n: \cup_{i=1}^n \gL_i = \gX$ for some $n \in \sZ_{>0}$, such that the likelihood ratio within each region $\gL_i$ is a constant $\eta_i \in [0, \infty)$:
$\eta_{\vx, \bar \vx}(\vz) = \eta_i, \forall \vz \in \gL_i$,
then we can sort the regions such that $\eta_1 \geq \eta_2 \geq \dots \geq \eta_n$. Note that $\gX$ can still be uncountable (see example in \xref{sec:warmup}). Then,
\begin{lemma}
\label{thm:main}
Let
$H^* \triangleq \argmin_H \bigg[ \sum_{i=1}^H \Pr(\rand(\vx) \in \gL_i) \geq p \bigg],$
then $\eta_{H^*}>0$, any $f^*$ satisfying Eq.~(\ref{eqn:optimal_f}) is a minimizer of Eq.~(\ref{eqn:target}). 
\begin{align}
    \forall i \in [n], \forall \vz \in \gL_i, & \Pr(f^*(\vz) = c) =\begin{cases}
         1,  &\text{if } i < H^*\\
        \frac{p - \sum_{i=1}^{H^*-1} \Pr(\rand(\vx) \in \gL_i)}{\Pr(\rand(\vx) \in \gL_{H^*})},  &\text{if } i = H^*\\
         0, &\text{if } i > H^*
        \end{cases}, \label{eqn:optimal_f}
\end{align}
and
$\rho_{\vx, \bar \vx,\gF}(p)
    = \sum_{i = 1}^{H^* - 1} \Pr(\rand(\bar \vx) \in \gL_i) + (p - \sum_{i=1}^{H^*-1} \Pr(\rand(\vx) \in \gL_i)) / \eta_{H^*}$
% \begin{align}
    % $\rho_{\vx, \bar \vx,\gF}(p)
    % = \sum_{i = 1}^{H^*} \frac{1}{\eta_i} \Pr(\rand(\vx) \in \gL_i) \one^*(i)$ %\label{eq:min_solution}
% \end{align}
\end{lemma}

We defer all the proofs to Appendix \ref{sec:proof-thm1}.


The minimization problem is essentially solved via the likelihood ratio testing~\cite{neyman1933ix}, by casting $\Pr(\phi(\vx) = \vz)$ and $\Pr(\phi(\bar \vx) = \vz)$ as likelihoods for two hypothesis with the significance level $p$.
The prior art~\cite{cohen2019certified} exploits the Neyman-Pearson lemma~\cite{neyman1933ix} to construct the bound for an isotropic Gaussian perturbation, but we will show that a stronger test is needed to solve Eq.~(\ref{eqn:target}) in some cases.

% (see Lemma 3 of \cite{cohen2019certified}) 
\begin{remark}
The Neyman-Pearson Lemma~\cite{neyman1933ix} does not suffice to solve Eq.~(\ref{eqn:target}) since it can only assign a deterministic prediction across each region with a distinct likelihood ratio. Its extension~\cite{tocher1950extension} to randomized tests also does not suffice since it assumes a countable $\gX$.
% with the main difference that our theorem considers the situation of setting partial probabilities for measure non-zero regions (when $i=H^*$). This turns out to be an important case in the discrete setting, see Algorithm \ref{alg} in Section \ref{sec:l0-perturb}.
\end{remark}

\begin{remark}
$\rho_{\vx, \bar \vx,\tilde{\gF}}(p)$  is an increasing continuous function of $p$; if $\eta_1 < \infty$, $\rho_{\vx, \bar \vx,\tilde{\gF}}(p)$ is a strictly increasing continuous function of $p$; if $\eta_1 < \infty$ and $\eta_n > 0$, the range of $\rho_{\vx, \bar \vx,\tilde{\gF}}(p)$ is $[0, 1]$.
% Among the $p$ values such that $\eta_{H^*} < \infty$, there is a strictly increasing bijection between $p$ and Eq.~(\ref{eq:min_solution}), which implies that if $ \eta_n < \infty$, there exists $\hat p \in [0, 1]$ such that $\forall p > \hat p,$ the solution to Eq.~(\ref{eq:min_solution}) is greater than $0.5$. 
% \label{rmk:bijection}
\end{remark}

\begin{corollary}
If $\eta_1 < \infty$ and $\rho_{\vx, \bar \vx,c}^{-1}(0.5) \neq \varnothing$, $\rho_{\vx, \bar \vx,c}^{-1}(0.5) = \min_{\{p \in [0, 1]: p > p' \implies \rho_{\vx, \bar \vx,c}(p') > 0.5\} } p$; moreover, if $\eta_1 < \infty$ and $\eta_n > 0$, $\rho_{\vx, \bar \vx,c}^{-1}(0.5) \neq \varnothing$.
% If $ \eta_n < \infty$ and $\eta_1 > 0$, 
% the minimizing $\hat p \in [0, 1]$ such that $p > \hat p$ implies the solution to Eq.~(\ref{eq:min_solution}) greater than $0.5$ is found by the inverse function of Eq.~(\ref{eq:min_solution}). 
\label{rmk:bijection}
\end{corollary}
% Hence, if $\eta_1 < \infty$ and $\eta_n > 0$, $\Pr(f(\phi(\vx))= c) > \rho_{\vx, \bar \vx,\tilde{\gF}}^{-1}(0.5) \implies \Pr(f(\phi(\bar \vx))= c) > 0.5$. 

% \ghl{not sure whether to mention the above commented part.}

Corollary~\ref{rmk:bijection} will be used in \xref{sec:l0-perturb} to derive efficient robustness certificates for an actual example.
Based on the overall results, we will show how to derive robustness guarantees in accuracy and AUC.

\subsection{Region-wise Robustness Certificates and Certified Accuracy}

We can extend $\rho_{\vx, \bar \vx, c}(p)$ (i.e., Eq.~(\ref{eqn:target})) by examining the worst case prediction probability over the neighboring region around $\vx$ to have a region-wise certificate. We expand the region until the worst case prediction falls below $0.5$, which yields the largest region that guarantees the classification of $c$. 

Formally, given an $\ell_q$ metric $\|\cdot\|_q$, the neighborhood around $\vx$ with radius $r$ is defined as $\gB_{r, q}(\vx) \triangleq \{\bar \vx \in \gX: \| \vx - \bar \vx \|_q \leq r\}$. Assuming $p = \Pr(f(\rand(\vx)) = c) > 0.5$ for a $c \in \gC$, the radius of the largest region that yields robust classification with respect to the class $c$ can be found by 
\begin{align}
    R(\vx, p, c, q) \triangleq \sup r, \text{  }s.t. \min_{\bar{\vx} \in \gB_{r, q}(\vx)}
    \rho_{\vx, \bar \vx, c}(p)  > 0.5. 
    \label{eq:main_lemma}
\end{align}
% Here $R(\vx, p, \gF, q)$ is tight in the sense that for any given $\vx, p, \gF, q$, and any  $r'>R(\vx, p, \gF, q)$, there exists $f'\in \gF, \|\vdel\|_q\in [R(\vx, p, \gF, q), r')$ such that $\Pr(f'(\rand(\vx)) = c)=p$, but $\Pr(f'(\rand(\vx + \vdel)) = c)\leq 0.5$.
Note that here we assume $\Pr(f(\rand(\vx)) = c) > 0.5$ and ignore the possibility of a correct prediction with $\Pr(f(\rand(\bar \vx)) = c) \leq 0.5$ for some $\bar \vx: \|\vx - \bar \vx\|_q > R(\vx, p, \gF, q)$.
Hence, the resulting radius is tight for binary classification, and a reasonable sufficient condition to guarantee robustness for $|\gC| > 2$. 
A tight guarantee will involve the maximum prediction probability over all the remaining classes (see Theorem 1 of \citep{cohen2019certified}). 
% which is statistically challenging to compute 
However, when the prediction probability $p = \Pr(f(\rand(\vx)) = c)$ relies on statistical estimation for each class $c$ (e.g., when $f$ is a deep network), the tight guarnatee is statistically challenging to obtain. 
The implementation of \citep{cohen2019certified} is also a special case of Eq.~(\ref{eq:main_lemma}).

The region-wise robustness certificates can be exploited to compute several measures. For example, we can compute the guaranteed accuracy when the adversary is restricted within an $\ell_q$ radius $r$:
\begin{align}
    ACC@r \triangleq \sum_{i=1}^N \one\{R(\vx_i, \Pr(f(\phi(\vx_i))=y_i), y_i, q) > r\}.
\end{align}
In the cases when the desired radius $r$ is unclear, we may evaluate the averaged radius $R(\vx_i, \Pr(f(\phi(\vx_i))=y_i), y_i, q)$ across the testing set, which can be realized as the area under guaranteed accuracy - radius curve. 

\subsection{Robustness Certificates in AUC}

In binary classification tasks, when the label distribution is unbalanced, AUC is a more appropriate measurement to evaluate the model than accuracy, since AUC considers the ranking of the prediction scores between the positive and the negative instances. 
If we denote the first $N_1$ out of $N$ instances as positive example, AUC can be computed as
\begin{align}
    \frac{1}{N_1(N-N_1)} \sum_{i=1}^{N_1}\sum_{j=N_1+1}^N S(\Pr(f(\phi(\vx_i))=1), \Pr(f(\phi(\vx_j))=1)), S(a, b) = \begin{cases}
    1,   &\;\text{if } a > b\\
    1/2, &\; \text{if } a=b\\
    0,   &\; \text{otherwise}
    \end{cases}.\nonumber
\end{align}
Measuring the guaranteed AUC under adversaries is slightly more involved than the case of accuracy, since the probability score of a positive instance impacts the evaluation of negative instance, and vice versa. 
However, the impact is always monotone in terms of the comparison function $S(\cdot, \cdot)$: for a positive instance $\vx_i$, the AUC score always monotonically decrease if we decrease the probability score of $\Pr(f(\phi(\vx_i))=1)$ regardless of the probability scores of the negative instances. Similar monotone property also holds for the negative instances. Hence, to maximally decrease the AUC score, we simply compute
$\min_{\bar \vx_i \in \gB_{r, q}(\vx_i)} \rho_{\vx_i, \bar \vx, y_i}$ for a point of interest $(\vx_i, y_i)$.

\ghl{Need some work to revise again...}
% \end{align}

% In the previous section, we have seen how to compute the certified radius for each data point $\vx$, which in turn tells us the certified accuracy under different perturbation radius. The certified accuracy is ``easy'' in the sense that the certified radius of each $\vx$ can be computed independently, and the final accuracy is a linear summation of the results of all data points. 

% For computing certified AUC, this linear summation idea does not work. As we see in (\ref{def:auc}), the AUC definition depends on the relative relationship between the scores of positive class and negative class, which is highly nonlinear. 

% The problem is simpler, if one can adversarially perturb \emph{all} the data points within certain fixed radius. In that case, we just apply Theorem \ref{thm:main} to compute the worst case score for every data points, and use (\ref{def:auc}) to compute the new robust AUC score. As a side note, since here we care about false positive rate and true positive rate, for the negative instances, we are not minimizing the probability of predicting negative in (\ref{eqn:target}). Instead, we are maximizing the probability of predicting positive for those instances, which is in fact equivalent. 

% Unfortunately, as we will see in Section \ref{sec:exp}, after perturbing all of the data points, the final robust AUC easily decreases  below $0.5$. Since random prediction already has AUC equal to $0.5$, such robust AUC certificate is meaningless. This is not surprising, since AUC depends on the relationship between positive and negative instances, so by adversarially perturbing all of them, the impact on AUC is much more than that on accuracy. 

% Before having a super strong model which can produce large robust AUC scores under the worst perturbation, an intermediate step would be to estimate the robust AUC score in a restricted setting. In the restricted setting, one can only perturb a fixed number of data points in order to minimize the AUC. But na\"{i}ve searching for the worst perturbation set of data points is computationally difficult. 

% By writing the problem as a quadratic program, we can solve this problem efficiently, as we show in Appendix \ref{sec:qp}. 


% We assume that the input data lie in the domain $\gX \subseteq \sR^D$, the output data lie in the target set $\gC$.
% In this paper, we adopt a random perturbation function $\rand$ to input  $\vx\in \gX$, which assigns a probability mass/density $\Pr(\rand(\vx) = \vz)$ for each perturbed outcome $\vz \in \gX$. 
% A simple example would be 
% % $\gX = \sR^d$, and 
% $\rand(\vx) = \vx+ \veps$ with $\veps \sim \gN(0, I)$~\cite{cohen2019certified}.
% % , but more general random transformations can also be used, as we will see later. 
% Therefore, $f(\rand(\vx))$ represents a probability distribution over $\gC$, rather than a deterministic value. 

% We denote the set of all possible measurable functions $\tilde \gF_{\gX, \gC}\triangleq \{f: f\in \gX\rightarrow \gC\}$, and the set of candidate functions for our task $\gF_{\gX, \gC}\subseteq \tilde \gF_{\gX, \gC}$. When $\gX, \gC$ are clearly defined, we drop the subscripts for $\gF_{\gX, \gC}$ and $\tilde \gF_{\gX, \gC}$ for notational simplicity.
% We denote the $\ell_q$-norm ball with radius $r$ around $\vx$ as $\gB_{r, q}(\vx) \triangleq \{\bar \vx \in \gX: \|\bar \vx - \vx\|_q \leq r\}$.


% Given two points $\vx, \bar \vx \in \gX$, for any point $\vz \in \gX$, denote the likelihood ratio $\eta_{\vx, \bar \vx}(\vz)\triangleq \Pr(\rand(\vx) = \vz)/\Pr(\rand(\bar \vx) = \vz)$. 
% To simplify the notation, 
% below we drop the subscripts of $\eta$ as $\vx, \bar \vx$ are always clearly defined. If $\gX$ is discrete, 
% we can split it into $n$ disjoint regions $\gL_1,\dots,\gL_n: \cup_{i=1}^n \gL_i = \gX$ such that the likelihood ratio within each region is a constant $\eta_i$: $\forall i \in [n], \vz \in \gL_i, \eta(\vz) = \eta_i$. 
% In this case, we can sort the regions by the likelihood ratio such that $\eta_1 \geq \eta_2 \geq \dots \geq \eta_n\geq 0$.

% =============== back up ===============

% \begin{theorem}
% \label{thm:main}
% % If $\gF$ is the set of all measurable functions with respect to $\rand$, and the cardinality of nonempty likelihood regions $N$ is finite, 
% % In the discrete case, if one considers all possible functions $\bar \gF$, we have a well structured solution for $\rho_{\vx, \bar \vx,\gF}(p)$ based on likelihood ratio $\eta$, see below. The continuous case is similar, which we omit here. 
% If $\gF=\tilde \gF$, based on sorted likelihood ratio $\eta_i$ and corresponding region $\gL_i$,
% define 
% $$H^* \triangleq \argmin_H \bigg[ \sum_{i=1}^H \Pr(\rand(\vx) \in \gL_i) \geq p \bigg],$$  
% Then $\eta_{H^*}>0$. 
% Define function $\one^*(i)\in [n]\rightarrow [0,1]$ as
% \begin{align}
%     & \one^*(i) =\begin{cases}
%          1,  &\text{if } i < H^*\\
%         \frac{p - \sum_{i=1}^{H^*-1} \Pr(\rand(\vx) \in \gL_i)}{\Pr(\rand(\vx) \in \gL_{H^*})},  &\text{if } i = H^*\\
%          0, &\text{if } i > H^*
%         \end{cases} \nonumber
% \end{align}
% Then we have
% \begin{align}
%     \rho_{\vx, \bar \vx,\gF}(p) %\triangleq \min_{\bar f \in \gF: \Pr(\bar f(\rand(\vx)) = c) = p} & \Pr(\bar f(\rand(\bar \vx)) =  c)  
%     = \sum_{i = 1}^{H^*} \frac{1}{\eta_i} \Pr(\rand(\vx) \in \gL_i) \one^*(i) \label{eq:min_solution}
% \end{align}
% And the corresponding minimizer $f^*$ is defined as:
% \begin{align*}
% \Pr(f^*(\vz) = c) = \one^*(i), \forall \vz \in \gL_i, i\in [n]
% \end{align*}
% \end{theorem}


% \subsection{Robustness Certificates of the Accuracy}

% for the  relationship between the prediction of $\vx$ and $\bar \vx$, we get the following lemma, stating that the robust radius of a given point $\vx$ is controlled by $\rho_{\vx, \bar \vx,\gF}(p)$.
% \begin{lemma}[Certified Radius]
% \label{lem:r-range}
% $\forall \vx \in \gX, f \in \mathcal{F}$, if there exists $ c\in \gC$, such that 
% $
% p \triangleq \Pr(f(\rand(\vx)) = c) > 0.5$, and 
% \begin{align}
%     R(\vx, p, \gF, q) \triangleq \sup r, \text{  }s.t. \min_{\bar{\vx} \in \gB_{r, q}(\vx)}
%     \rho_{\vx, \bar \vx,\gF}(p)  > 0.5. 
%     \label{eq:main_lemma}
% \end{align}
% Then $\Pr(f(\rand(\vx + \vdel)) = c) > 0.5$ whenever $\|\vdel\|_q < R(\vx, p, \gF, q)$ and $\vx + \vdel \in \gX$. The bound $R(\vx, p, \gF, q)$ is tight in the sense that 
% for any given $\vx, p, \gF, q$, and any  $r'>R(\vx, p, \gF, q)$, 
% there exists $f'\in \gF, \|\vdel\|_q\in [R(\vx, p, \gF, q), r')$ such that 
% $\Pr(f'(\rand(\vx)) = c)=p$, but 
% $\Pr(f'(\rand(\vx + \vdel)) = c)\leq 0.5$.
% %  the $\ell_q$-norm of perturbations and the existence of $\bar{f} \in \gF$ that constitutes violation.
% % \footnote{Note that, to simplify notation, we drop the dependency of $\gF$, $\gX$, $\ell_q$-norm, and $p$ in the notation of $R(\vx)$.}  
% \label{lem:clean_general}
% \end{lemma}

% \begin{proof}
% \textbf{Sufficiency}: Let $r \triangleq \| \vdel \|_q < R(\vx, p, \gF, q)$ and $\vx + \vdel \in \gX$, then $\vx+\vdel \in \gB_{r, q}(\vx)$.
% \begin{align}
%     \Pr(f(\rand(\vx + \vdel)) = c) \geq \min_{\bar{\vx} \in \gB_{r, q}(\vx) } \rho_{\vx, \bar \vx,\gF}(p)  > 0.5, \nonumber
% \end{align}
% where the last inequality holds by the definition of $R(\vx, p, \gF, q)$.

% \textbf{Necessity}:
% for any given $\vx, p, \gF, q$, and any  $r'>R(\vx, p, \gF, q)$, 
% if for all $\vdel$ such that  $\|\vdel\|_q\in [R(\vx, p, \gF, q), r')$, $\rho_{\vx, \vx+\vdel,\gF}(p) > 0.5$, 
% then it means
% \begin{align}
%     \forall r<r', \text{  } \min_{\bar{\vx} \in \gB_{r, q}(\vx)}
%     \rho_{\vx, \bar \vx,\gF}(p)  > 0.5. 
% \end{align}
% This contradicts the definition of  $R(\vx, p, \gF, q)$.
% \end{proof}
% % When defining $R(\vx, p, \gF, q)$, we are enumerating all possible functions in $\gF$. This immediately gives us the following corollary. 
% % \begin{corollary}
% % The bound is tight with respect to a functional class $\gF$; the smaller the functional class $\gF$ is identified, the tighter bound is obtained. That means, $\gF \subseteq \gF' \implies R(\vx, p, \gF, q) \geq R(\vx, p, \gF', q)$.
% % \label{rmk:tight}
% % \end{corollary}

% % Later in Section \ref{sec:examples}, we will see examples of applying our Lemma \ref{lem:r-range} and Corollary \ref{rmk:tight} to get better robustness certificates. 


% % where we may say
% % \begin{align}
% %     \baserand(\vx_i) = \vx_i + \veps_i, \veps_i \overset{i.i.d.}{\sim} \gN(0, \sigma^2), \forall i \in [d]
% % \end{align}
% % for a given $\sigma$. 



% \subsection{Robustness Certificates of the AUC}
% In the previous section, we have seen how to compute the certified radius for each data point $\vx$, which in turn tells us the certified accuracy under different perturbation radius. The certified accuracy is ``easy'' in the sense that the certified radius of each $\vx$ can be computed independently, and the final accuracy is a linear summation of the results of all data points. 

% For computing certified AUC, this linear summation idea does not work. As we see in (\ref{def:auc}), the AUC definition depends on the relative relationship between the scores of positive class and negative class, which is highly nonlinear. 

% The problem is simpler, if one can adversarially perturb \emph{all} the data points within certain fixed radius. In that case, we just apply Theorem \ref{thm:main} to compute the worst case score for every data points, and use (\ref{def:auc}) to compute the new robust AUC score. As a side note, since here we care about false positive rate and true positive rate, for the negative instances, we are not minimizing the probability of predicting negative in (\ref{eqn:target}). Instead, we are maximizing the probability of predicting positive for those instances, which is in fact equivalent. 

% Unfortunately, as we will see in Section \ref{sec:exp}, after perturbing all of the data points, the final robust AUC easily decreases  below $0.5$. Since random prediction already has AUC equal to $0.5$, such robust AUC certificate is meaningless. This is not surprising, since AUC depends on the relationship between positive and negative instances, so by adversarially perturbing all of them, the impact on AUC is much more than that on accuracy. 

% Before having a super strong model which can produce large robust AUC scores under the worst perturbation, an intermediate step would be to estimate the robust AUC score in a restricted setting. In the restricted setting, one can only perturb a fixed number of data points in order to minimize the AUC. But na\"{i}ve searching for the worst perturbation set of data points is computationally difficult. 

==> old.tex <==
\section{\textred{Previous results, don't look at this}}
































For each $v$ and $\alpha$, we can compute the strict lower bound on $p$ where the $p$ has to be strictly higher than the value in order to have the guarantee. 


\begin{prop}
We assume $\gF$ is the set of all measurable functions with respect to $Z$. 
% If the range of $Z$ is $\gX$ with $\Pr(Z(\vx) = \vz) > 0$ everywhere for all $\vx \in \gX$, the minimum of Eq.~(\ref{eq:main_lemma}) given a fixed $\bar{\vx}$ is
\begin{align}
    \int^{\infty}_H \Pr(Z(\vx) \in \gX(\eta, \vx, \bar{\vx})) \mathrm{d}\eta \nonumber
\end{align}
is a continuous function of $H \in [0, \infty)$ for fixed $\vx$ and $\bar \vx$, the minimum and minimizer of Eq.~(\ref{eq:main_lemma}) for the $\vx$ and $\bar{\vx}$ is
\begin{align}
    \min_{\bar f \in \gF: \Pr(\bar f(Z(\vx)) = c) = p} \Pr(\bar f(Z(\bar \vx)) = & c)  
    = \int^\infty_{H^*} \frac{1}{\eta} \Pr(Z(\vx) \in \gX(\eta, \vx, \bar{\vx})) \mathrm{d}\eta \nonumber \\
    \argmin_{\bar f \in \gF: \Pr(\bar f(Z(\vx)) = c) = p} \Pr(\bar f(Z(\bar \vx)) = & c) 
    = f^*: \begin{cases}
        f^*(\vz) = c,  &\text{if } \Pr(Z(\vx) = \vz) / \Pr(Z(\bar \vx) = \vz) \geq H^*,\\
        f^*(\vz) \neq c, &\text{if } \Pr(Z(\vx) = \vz) / \Pr(Z(\bar \vx) = \vz) < H^*,
        \end{cases} \nonumber \\
    & \text{where  }H^* = \argmax_H \int^{\infty}_H \Pr(Z(\vx) \in \gX(\eta, \vx, \bar{\vx})) \mathrm{d}\eta = p. \nonumber
\end{align}
\end{prop}

\begin{proof}
We can decompose the integral on $\gX$ among each region with different likelihood ratio, which is valid since the integral is bounded by $1$. It yields
\begin{align}
    \Pr(\bar f(Z ( \vx)) = c) = \int^\infty_0 \int_{\vz \in \gX(\eta, \vx, \bar \vx)} \Pr(Z(\vx) = \vz) \Pr(\bar f(\vz) = c) \mathrm{d}\vz \mathrm{d}\eta,
\end{align}
and 
\begin{align}
    \Pr(\bar f(Z (\bar \vx)) = c) & = \int^\infty_0 \int_{\vz \in \gX(\eta, \vx, \bar \vx)} \Pr(Z(\bar \vx) = \vz) \Pr(\bar f(\vz) = c) \mathrm{d}\vz \mathrm{d}\eta. \\
    & = \int^\infty_0 \frac{1}{\eta} \int_{\vz \in \gX(\eta, \vx, \bar \vx)} \Pr(Z( \vx) = \vz) \Pr(\bar f(\vz) = c) \mathrm{d}\vz \mathrm{d}\eta.
\end{align}
To simplify notation, we denote 
\begin{align}
    \Pr(\bar f(\gX(\eta, \vx, \bar \vx)) = c) \triangleq \int_{\vz \in \gX(\eta, \vx, \bar \vx)} \Pr(Z(\vx) = \vz) \Pr(\bar f(\vz) = c) \mathrm{d}\vz. 
\end{align}
Then the minimization problem can be rewritten as

\begin{align}
    \min & \int_{0}^\infty \frac{1}{\eta} \Pr(\bar f(\gX(\eta, \vx, \bar \vx)) = c) \mathrm{d} \eta \\
    \text{s.t. } & \int_{0}^\infty \Pr(\bar f(\gX(\eta, \vx, \bar \vx)) = c) \mathrm{d} \eta = p.
\end{align}

\textred{TBD: continue with Lemma 5.} 
\end{proof}


\begin{remark}
(Informal) Given a $\bar{\delta}$, the minimum of $\bar{f}$ in Eq.~(\ref{eq:main_lemma}) can be found by putting the function values $\bar{f}(\vz) = c$ in the order of decreasing likelihood ratio $\Pr(\vz = \epsilon) / \Pr(\vz = \bar{\delta} + \epsilon)$ of $\vz \in \sR^d$.
\end{remark}

\textred{Maybe replace the above lemma with an actual equation showing the summation/integral on the likelihood ratio...}


Solving the minimax problem for each $\vx$ with possibly different $p$ can be time-consuming. An alternative way is to specify a fixed $r$, and ask whether $R(\vx, p, \gF, q) \geq r$. When the range of $Z$ is equal to $\gX$ with positive density/mass everywhere, we have a strictly increasing bijection between $p$ and 
\begin{align}
    \min_{\substack{\bar{\vx} \in \gX \cap \gB_{r, q}(\vx) \\ \bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(\vx)) = c) = p}}
    \Pr(\bar{f}(Z(\bar{\vx})) = c).
\end{align}
Hence, we can first compute the mini

\subsection{A Discrete Perturbation}

% In the remaining paper, we are in general interested in an cooridinate-wise random transformation:
% \begin{align}
%     Z(\vx) = Z(\vx_1,\dots,\vx_d) = [\baserand(\vx_1),\dots,\baserand(\vx_d)],
% \end{align}
% where we may say
% \begin{align}
%     \baserand(\vx_i) = \vx_i + \epsilon_i, \epsilon_i \overset{i.i.d.}{\sim} \gN(0, \sigma^2), \forall i \in [d]
% \end{align}
% for a given $\sigma$. 

In this section, we are interested in the data space $\gX = \{0, 1/K, \dots, 1\}^d \triangleq \{K\}^d$ and the following distribution:
\begin{align}
    \sZ \begin{cases}
    \Pr(\baserand(\vx_i) = \vx_i) = \alpha, &\\
    \Pr(\baserand(\vx_i) = z) = (1-\alpha) / K \triangleq \beta, &\text{if } z \in \{K\}: z \neq \vx_i,
    \end{cases}
\end{align}
which can be regarded as a mixture between a delta function and a uniform distribution with a parameter $\alpha$. To solve the minimax problem in Lemma~\ref{lem:clean_general}, we first observe that for each $\ell_0$-norm $r \in \sZ_{>0}$, there are at most $(d+1)^2$ regions with different likelihood ratios: given $\vx \in \gX$ for every possible transformation $\vz \in \gX$, the likelihood for such transform is one of the following $d+1$ choices: $\alpha^d, \alpha^{d-1} \beta, \dots,\alpha\beta^{d-1}, \beta^d$. Similarly, the likelihood for the transformation of an $\bar{\vx} \in \gX: \|\bar{\vx} - \vx\|_0 \leq r$ also has $d+1$ choices. 

During inference, we may solve the minimax problem for each $\vx$ separately. However, i

We may solve the minimax problem in the following way: given $p$ and $r = 1, 2, ...$, we compute the minimization problem:
\begin{align}
    \min_{\substack{\bar{\vx} \in \gX: \|\bar{\vx} - \vx\|_q = r \\ \bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(\vx)) = c) = p}}
    \Pr(\bar{f}(Z(\bar{\vx})) = c)
\end{align}
and check when the value is lower than $0.5$.

By the uniformity of the distribution, we know every $\bar{\vx}$ is the same in terms of perturbation from $\vx$ given the same $\ell_0$ distance. WLOG, we may assume $\vx = [0, \dots, 0]$, and $\bar{\vx} = \bar{\delta}_v \triangleq [1, \dots, 1, 0, \dots, 0]$ with $v$ $1$s and $d-v$ $0$s for computing the optimum,
\begin{align}
    \min_{\substack{\bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(0)) = c) = p}}
    \Pr(\bar{f}(Z(\bar{\delta}_v)) = c),
\end{align}
and check when the value is lower than $0.5$.

We use the likelihood ratio $\frac{\alpha^{d-m} \beta^{m}}{\alpha^{d-n} \beta^{n}}$ to refer the scenario when $\vx$ flips $m$ coordinates, and $\bar \vx$ flips $n$ coordinates. For $v \in [d]$ and $(m, n) \in \{0, 1, \dots, d\}^2$, the number of possible outcome $\vx' \in \gX$ with likelihood ratio can be computed in the following way:
\begin{align}
    \#(m, n) = \sum_{i=0}^{\min(m, d-v)} \sum_{j=0}^{m-i}  \frac{(K - 1)^j \one((m-i-j) + (n-i-j) + j = v) v !}{(m-i-j)!(n-i-j)!j!} \frac{K^i(d - v)!}{(d-v-i)! i!}, \forall n, m \in \lfloor d \rfloor, m \leq n, \label{eq:compute:init:2}
\end{align}
where the first summation corresponds to the case where $i$ bits in the last $(d-v)$ dimensions are flipped, and the second summation corresponds to the case where $j$ bits in the first $v$ dimensions are flipped to any value other than $\{0, 1\}$, $m - i - j$ bits in $\vx$ are flipped to $1$, and $n - i - j$ bits in $\bar \vx$ are flipped to $0$. The indicator function verifies that whether the value of $j$ is valid. If we let $j^* \triangleq m + n - 2i - v$, we have
\begin{align}
    (\ref{eq:compute:init:2}) = & \sum_{i=0}^{\min(m, d-v)} \frac{\one(j^* \geq 0) \one(j^* \leq m-i) (K - 1)^{j^*} v !}{(m-i-j^*)!(n-i-j^*)!j^*!} \frac{K^i(d - v)!}{(d-v-i)! i!}, \forall n, m \in \lfloor d \rfloor, m \leq n, \\
    & = \sum_{i=\max\{0, n - v\}}^{\min(m, d-v)} \frac{\one(j^* \geq 0) (K - 1)^{j^*} v !}{(m-i-j^*)!(n-i-j^*)!j^*!} \frac{K^i(d - v)!}{(d-v-i)! i!}, \forall n, m \in \lfloor d \rfloor, m \leq n, \\
    & = \sum_{i=\max\{0, n - v\}}^{\min(m, d-v, \lfloor \frac{m+n-v}{2} \rfloor )} \frac{(K - 1)^{j^*} v !}{(m-i-j^*)!(n-i-j^*)!j^*!} \frac{K^i(d - v)!}{(d-v-i)! i!}, \forall n, m \in \lfloor d \rfloor, m \leq n, \\ \label{eq:compute:2nd:2}
\end{align}
We also know $\#(m, n) = \#(n, m)$.

For each $v$ and $\alpha$, we can compute the strict lower bound on $p$ where the $p$ has to be strictly higher than the value in order to have the guarantee. 



\section{The general lemma}

\header{Notations}
\begin{enumerate}
    \item We have noise $\epsilon \sim \gP$ according to a distribution $\gP$.
    \item $\gF$ is the set of measurable functions w.r.t. $\gP$.
    \item The label class is denoted as $c \in \gC$. 
\end{enumerate}

\begin{lem}
$\forall \vx \in \sR^d, f \in \mathcal{F}$, with $p \triangleq \Pr(f(\vx + \epsilon) = c) > 0.5$, and we define
\begin{align}
    % R(\vx, p) & = \sup v \\
    R(\vx, p) \triangleq \sup v, \text{  }s.t. \min_{\substack{\bar{\delta} \in \sR^d: \|\bar{\delta}\|_q \leq v \\ \bar{f} \in \mathcal{F}: \Pr(\bar{f}(\vx + \epsilon) = c) = p}}
    % s.t. & \inf_{\delta \in \sR^d: \|\delta\|_q \leq v} \inf_{\bar{f} \in \mathcal{F}: \Pr(\bar{f}(\vx + \epsilon) = c) = p}
    % \Pr(\bar{f}(\vx + \bar{\delta} + \epsilon) = c) > 0.5. \label{eq:main_lemma}
    % s.t. & \inf_{\bar{f} \in \mathcal{F}: \sP_{\epsilon}(\bar{f}(\vx + \epsilon) = c) = p} \sP_{\epsilon}(\bar{f}(\vx + \delta + \epsilon) = c) > 0.5.
\end{align}
Then $\Pr(f(\vx + \delta + \epsilon) = c) > 0.5$ whenever $\|\delta\|_q < R(\vx, p)$, and the bound $R(\vx, p)$ is tight in term of both the $\ell_q$-norm of perturbations and the existence of $\bar{f} \in \gF$ that constitutes violation.  
\end{lem}

\begin{proof}
If $\| \delta \|_q < R(\vx, p)$, 
\begin{align}
    \Pr(f(\vx + \delta + \epsilon) = c) \geq \min_{\substack{\bar{\delta} \in \sR^d: \|\bar{\delta}\|_q \leq v \\ \bar{f} \in \mathcal{F}: \Pr(\bar{f}(\vx + \epsilon) = c) = p}} \Pr(\bar{f}(\vx + \bar{\delta} + \epsilon) = c) > 0.5. \nonumber
\end{align}
If $\| \delta \|_q > R(\vx, p)$, $\exists \bar{\delta} \in \sR^D: \| \delta \|_q > \|\bar{\delta}\|_q > R(\vx, p)$ s.t.
\begin{align}
    & \min_{\bar{f} \in \mathcal{F}: \Pr(\bar{f}(\vx + \epsilon) = c) = p} \Pr(\bar{f}(\vx + \bar{\delta} + \epsilon) = c) \leq 0.5,
    \text{ and } 
    \exists \bar{f} \in \gF: \Pr(\bar{f}(\vx + \bar{\delta} + \epsilon) = c) \leq 0.5; \nonumber
\end{align}
otherwise, it will lead to contradiction. 
\end{proof}

\begin{remark}
The bound is tight with respect to a functional class $\gF$, so one may use a subset $\gF' \subset \gF$ to derive a similar but possibly smaller bound, which is tight with respect to $\gF'$ but not $\gF$. 
\end{remark}

\begin{remark}
(Informal) Given a $\bar{\delta}$, the minimum of $\bar{f}$ in Eq.~(\ref{eq:main_lemma}) can be found by putting the function values $\bar{f}(\vz) = c$ in the order of decreasing likelihood ratio $\Pr(\vz = \epsilon) / \Pr(\vz = \bar{\delta} + \epsilon)$ of $\vz \in \sR^d$.
\end{remark}

\section{l1 norm and the delta-uniform mixture distribution}

\update{[New General Lemma]}

Assume that the data lie in $\gX \subseteq \sR^d$, and we are given a randomized mapping $Z$ that assigns a probability density/mass for each possible outcome $\Pr(Z(\vx) = \vz), \vz \in \gX$. A basic realization of this scheme would be $\gX = \sR^d$, and $Z(\vx) = \epsilon + \vx$ with $\epsilon \sim \gN(0, I)$. Here we denote $\gF$ as the set of measurable functions w.r.t. the transformation $Z$, denote the set of class labels as $\gC$, and the $\ell_q$-norm ball with radius $v$ around $\vx$ as $\gB_{v, q}(\vx) \triangleq \{\bar \vx \in \sR^d: \|\bar \vx - \vx\|_q \leq v \}$

\begin{lem}
$\forall \vx \in \gX, f \in \mathcal{F}$, with $p \triangleq \Pr(f(Z(\vx)) = c) > 0.5$ for some $c \in \gC$, and we define
\begin{align}
    % R(\vx) \triangleq \sup v, \text{  }s.t. \min_{\substack{\bar{\vx} \in \gX: \|\bar{\vx} - \vx\|_q \leq v \\ \bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(\vx)) = c) = p}}
    R(\vx) \triangleq \sup v, \text{  }s.t. \min_{\substack{\bar{\vx} \in \gX \cap \gB_{v, q}(\vx) \\ \bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(\vx)) = c) = p}}
    \Pr(\bar{f}(Z(\bar{\vx})) = c) > 0.5. 
    % \label{eq:main_lemma}
\end{align}
Then $\Pr(f(Z(\vx + \delta)) = c) > 0.5$ whenever $\|\delta\|_q < R(\vx)$ and $\vx + \delta \in \gX$, and the bound $R(\vx)$ is tight in term of both the $\ell_q$-norm of perturbations and the existence of $\bar{f} \in \gF$ that constitutes violation.\footnote{Note that, to simplify notation, we drop the dependency of $\gF$, $\gX$, $\ell_q$-norm, and $p$ in the notation of $R(\vx)$.}  
\label{lem:new_general}
\end{lem}

\begin{proof}
If $v \triangleq \| \delta \|_q < R(\vx)$ and $\vx + \delta \in \gX$, 
\begin{align}
    \Pr(f(Z(\vx + \delta)) = c) \geq \min_{\substack{\bar{\vx} \in \gX \cap \gB_{v, q}(\vx) \\ \bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(\vx)) = c) = p}} \Pr(\bar{f}(Z(\bar{\vx})) = c) > 0.5, \nonumber
\end{align}
If $\| \delta \|_q > R(\vx)$, $\exists \bar{\delta} \in \sR^D: \| \delta \|_q > \|\bar{\delta}\|_q > R(\vx, p)$ and $\vx + \bar{\delta} \in \gX$ s.t.
\begin{align}
    & \min_{\bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(\vx)) = c) = p} \Pr(\bar{f}(Z(\vx + \bar{\delta})) = c) \leq 0.5,
    \text{ and } 
    \exists \bar{f} \in \gF: \Pr(\bar{f}(Z(\vx + \bar{\delta})) = c) \leq 0.5; \nonumber
\end{align}
otherwise, it will lead to contradiction. 
\end{proof}

\section{Uniform-Delta Mixture Distribution}

% In this section, we are interested in the following coordinate-wise identical and independent random transformation:
In the remaining paper, we will focus on cooridinate-wise i.i.d. random transformations:
\begin{align}
    Z(\vx) = Z(\vx_1,\dots,\vx_d) = [\baserand(\vx_1),\dots,\baserand(\vx_d)],
\end{align}
where we may say
\begin{align}
    \baserand(\vx_i) = \vx_i + \epsilon_i, \epsilon_i \overset{i.i.d.}{\sim} \gN(0, \sigma^2), \forall i \in [d]
\end{align}
for a given $\sigma$. In this section, we are interested in the data space $\gX = \{0, \dots, K\}^d \triangleq [K]^d$ and the following distribution:
\begin{align}
    \begin{cases}
    \Pr(\baserand(\vx_i) = \vx_i) = \alpha, &\\
    \Pr(\baserand(\vx_i) = z) = (1-\alpha) / K \triangleq \beta, &\text{if } z \in \{0, \dots, K\}: z \neq \vx_i,
    \end{cases}
\end{align}
which can be regarded as a mixture between a delta function and a uniform distribution with a parameter $\alpha$. To solve the minimax problem in Lemma~\ref{lem:new_general}, we first observe that for each $\ell_0$-norm $v \in \sZ_{>0}$, there are at most $(d+1)^2$ regions with different likelihood ratios: given $\vx \in \gX$ for every possible transformation $\vz \in \gX$, the likelihood for such transform is one of the following $d+1$ choices: $\alpha^d, \alpha^{d-1} \beta, \dots,\alpha\beta^{d-1}, \beta^d$. Similarly, the likelihood for the transformation of an $\bar{\vx} \in \gX: \|\bar{\vx} - \vx\|_0 \leq v$ also has $d+1$ choices. 

We may solve the minimax problem in the following way: given $p$ for $v = 1, 2, ...$, we compute the minimization problem:
\begin{align}
    \min_{\substack{\bar{\vx} \in \gX: \|\bar{\vx} - \vx\|_q = v \\ \bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(\vx)) = c) = p}}
    \Pr(\bar{f}(Z(\bar{\vx})) = c)
\end{align}

By the uniformity of the distribution, we know every $\bar{\vx}$ is the same in terms of perturbation from $\vx$ given the same $\ell_0$ distance. WLOG, we may assume $\vx = [0, \dots, 0]$, and $\bar{\vx} = \bar{\delta}_v \triangleq [1, \dots, 1, 0, \dots, 0]$ with $v$ $1$s and $d-v$ $0$s for computing the optimum,
\begin{align}
    \min_{\substack{\bar{f} \in \mathcal{F}: \Pr(\bar{f}(Z(0)) = c) = p}}
    \Pr(\bar{f}(Z(\bar{\delta}_v)) = c),
\end{align}
and check whether the value is greater than $0.5$ for each $v$. We use the likelihood ratio $\frac{\alpha^{d-m} \beta^{m}}{\alpha^{d-n} \beta^{n}}$ to refer the scenario when $\vx$ flips $m$ coordinates, and $\bar \vx$ flips $n$ coordinates. For $v \in [d]$ and $(m, n) \in \{0, 1, \dots, d\}^2$, the number of possible outcome $\vx' \in \gX$ with likelihood ratio can be computed in the following way:
\begin{align}
    \#(m, n) = \sum_{i=0}^{\min(m, d-v)} \sum_{j=0}^{m-i}  \frac{(K - 1)^j \one((m-i-j) + (n-i-j) + j = v) v !}{(m-i-j)!(n-i-j)!j!} \frac{K^i(d - v)!}{(d-v-i)! i!}, \forall n, m \in \lfloor d \rfloor, m \leq n, \label{eq:compute:init:3}
\end{align}
where the first summation corresponds to the case where $i$ bits in the last $(d-v)$ dimensions are flipped, and the second summation corresponds to the case where $j$ bits in the first $v$ dimensions are flipped to any value other than $\{0, 1\}$, $m - i - j$ bits in $\vx$ are flipped to $1$, and $n - i - j$ bits in $\bar \vx$ are flipped to $0$. The indicator function verifies that whether the value of $j$ is valid. If we let $j^* \triangleq m + n - 2i - v$, we have
\begin{align}
    (\ref{eq:compute:init}) = & \sum_{i=0}^{\min(m, d-v)} \frac{\one(j^* \geq 0) \one(j^* \leq m-i) (K - 1)^{j^*} v !}{(m-i-j^*)!(n-i-j^*)!j^*!} \frac{K^i(d - v)!}{(d-v-i)! i!}, \forall n, m \in \lfloor d \rfloor, m \leq n, \\
    & = \sum_{i=\max\{0, n - v\}}^{\min(m, d-v)} \frac{\one(j^* \geq 0) (K - 1)^{j^*} v !}{(m-i-j^*)!(n-i-j^*)!j^*!} \frac{K^i(d - v)!}{(d-v-i)! i!}, \forall n, m \in \lfloor d \rfloor, m \leq n, \\
    & = \sum_{i=\max\{0, n - v\}}^{\min(m, d-v, \lfloor \frac{m+n-v}{2} \rfloor )} \frac{(K - 1)^{j^*} v !}{(m-i-j^*)!(n-i-j^*)!j^*!} \frac{K^i(d - v)!}{(d-v-i)! i!}, \forall n, m \in \lfloor d \rfloor, m \leq n, \\ \label{eq:compute:2nd:3}
\end{align}
We also know $\#(m, n) = \#(n, m)$.

% The indicator is equivalent to 
% \begin{align}
%     \one(m +n - 2i = v + j) = \one((m-i-j) + (n-i-j) + j = v),
% \end{align}
% which checks whether such assignment is valid: there are $(m-i-j)$ bits in $\vx$ are flipped to $1$, $(n-i-j)$ bits in $\bar \vx$ are flipped to $0$, and the remaining $j$ bits are flipped to an arbitrary value, and we ensure that the number of bits sum to $v$.

% with a dynamic program on the number of data dimension $d$, the $\ell_0$ norm $v$, and the number of changes possible for $\vx$ and $\bar \vx$: $N[d, v, m, n]$.

% \begin{algorithm}
% \caption{Algorithm to find the possible number of outcomes for each likelihood ratio}\label{alg:euclid}
% \begin{algorithmic}[1]
% \Procedure{Count}{$d, m, n, v$}\Comment{return the possible outcome for $d$-dimensional inputs with $v$ $\ell_0$-norm w.r.t. likelihoods $m$ for $\vx$ and $n$ for $\bar \vx$}
% \If{($v = 0$ and $m\neq n$) or $\min\{m, n\} < 0$ or $\max\{m, n\} > d$ or $m+n < v$}\Comment{Early stopping.}
% \State{return $0$;}
% \EndIf

% \If{$d = 0$}
% \If{$m = 0$ and $n = 0$ and $v = 0$}
% \State{return $1$;}
% \Else
% \State{return $0$;}
% \EndIf
% \EndIf


% \If{$v = 0$}
% \State{return $(^d_m) \times K^m $;}
% \Comment{Put the current index as $0$ or any other value.}
% \Else
% \State{return Count($d-1, m-1, n, v-1$) + Count($d-1, m, n-1, v-1$) + $(K-1) \times$ Count($d-1, m-1, n-1, v-1$)}\Comment{Put the current index as $1, 0$ or any other value.}
% \EndIf
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

For each $v$ and $\alpha$, we can compute the strict lower bound on $p$ where the $p$ has to be strictly higher than the value in order to have the guarantee. 

% \begin{lem}
% For $v \in \sZ_{>0}$ and $(m, n) \in \{0, 1, \dots, d\}^2$, the volume of the region with likelihood ratio $\frac{\alpha^{d-m} \beta^{m}}{\alpha^{d-n} \beta^{n}}$ is XXX.
% \end{lem}

% \begin{proof}

% \header{Case 1.} If $m+n < v$, it impossible for $\vx$ and $\bar \vx$ to both reach it, thus the region is empty for $m+n < v$. Hence, we can only check for each $m \in \{v, v+1, \dots, n\}$

% \header{Case 2.} If $m < v, m+n \geq v$, 
% \begin{enumerate}
%     \item $n = v - m$, it has $(^v_m) = (^v_n)$ possible choices. 
%     \item $n = v - m + 1$, it is impossible for $\bar \vx$ to have anything other than $0$ for the $v+1^\text{th}$ to the last dimension. 
% \end{enumerate}

% \end{proof}

% , which can be either $[K]^d \triangleq \{0, \dots, K\}^d$ or $[0, K]^d$. 
% Given $\vx \in \gX$, we define a randomized transformation $Z$:
% \begin{align}
%     Z(\vx_1,\dots,\vx_d) = [\baserand(\vx_1),\dots,\baserand(\vx_d)] 
% \end{align}

% \begin{align}
%     \Pr(Z(\vx_1,\dots,\vx_d) | \vx; \alpha) = \prod_{i \in [d]} \Pr(\baserand(\vx_i)| \vx_i; \alpha) \triangleq \prod_{i \in [d]} \alpha^{\one(\baserand(\vx_i) = \vx_i)} (\frac{1 - \alpha}{K}) ^{\one(\baserand(\vx_i) = \vx_i)}.
% \end{align}
% We are interested in the variant:


\section{Current Idea}
Consider the Laplace distribution $P(x)=\frac{1}{(2b)^d} e^{-\frac{\|x\|_1}{b}}$ for $x\in \R^d$. We are interested in 
the smoothed classifier $g$, which returns whichever class the base classifier $f$ is most liklely to return when $x$ is perturbed by the noise sampled from $P$:
\begin{equation}
    g(x)\triangleq
    \argmax_{c\in Y}
    \Pr(f(x+\eps) = c), ~~~~~~~~\eps\sim P 
    \label{def:smoothed_output}
\end{equation}

That is, $g(x)$ will return class $c$ such that the decision region $\{x'\in \R^d: f(x')=c\}$ has largest measure under the distribution $P$. 

We have the following robustness guarantee: 

\begin{thm}
Let $f:\R^d \rightarrow Y$ be any deterministic or rnadom function, and let $\eps\sim P$. Let $g$ be defined as in (\ref{def:smoothed_output}). Suppose $\pa, \pb\in [0,1]$ are such that:
\[
\Pr(f(x+\eps)=c_A)\geq 
\pa\geq \pb \geq 
\max_{c\neq c_A} \Pr(f(x+\eps)=c)
\]
Then $g(x)=g(x+\delta)$ whenever $\|\delta\|_1<R$, where 
\[
R=- b \ln (2 - 2\pa) 
\]
\end{thm}

For simplicity, we assume that there are only two classes, i.e., $c_A$, and $c_B$. 
Without loss of generality, below we assume $x=0$. 
WLOG, assume $g(0)=c_A$, and $\Pr(f(\eps)=c_A)=\bar P>0.5$.

Define $\one(x)\triangleq \one(f(x)=c_A)$, that is, whether the output of the classifier $f$ on the point $x$ is $c_A$.  We have,
\begin{align}
 \bar P= \Pr(f(\eps)=c_A)
 &=
\int_{x\in \R^d} \one(x) P(x) dx\label{eqn:int_def_f_eps}
\end{align}

Given $\delta$, we know that $g(0)= g(\delta)$ if and only if $\Pr(f(\delta +\eps)= c_A)>0.5$. Below we show that if $\|\delta\|_1 \leq R<??$,  we have $\Pr(f(\delta +\eps)= c_A)>0.5$, which gives $g(0)= g(\delta)$. Moreover, this is also tight, as we will give one example showing that if $\|\delta\|_1 = R$, there exists a classifier $f$ such that $\Pr(f(\delta +\eps)= c_A)=0.5$. 



We would like to understand the following program: 
\begin{align}
\mathrm{(I)}\triangleq  
\min_{\delta:\|\delta\|_1=c }
\min_{\one(\cdot)}
~~&\int_{x\in \R^d}
\one(x)
P(x-\delta) dx
\label{eqn:target}
\\
s.t. ~~&
\int_{x\in \R^d}
\one(x)
P(x) dx=\bar P
\label{eqn:constraint}
\end{align}
 


Notice that $P(x)$ can be written as infinitely many $\ell_1$ balls stacked together:
\[
P(x)=\frac1{b(2b)^d}
\int_{r=\|x\|_1}^{\infty}
e^{-\frac{r}{b}}
dr
\]


In other words, program $\mathrm{(I)}$ can be written as, 
\begin{align*}
\mathrm{(I)}=\min_{\delta:\|\delta\|_1=c }
\min_{\one(\cdot)}
~~&
\frac1{b(2b)^d}
\int_{x\in \R^d}
\int_{r=\|x-\delta \|_1}^\infty 
\one(x)
e^{-\frac{r}{b}} dr dx\\
s.t. ~~&
\frac1{b(2b)^d}
\int_{x\in \R^d}
\int_{r=\|x \|_1}^\infty 
\one(x)
e^{-\frac{r}{b}} dr dx=\bar P
\end{align*}

We relax this program such that there are different indicator functions $\one_r(\cdot)$ for different radius $r$, and for all $x, r$, $\one_r(x)\in \{0, 1\}$. Therefore, when $\one_r(x)=\one(x)$ for all $r\in [0,\infty)$, it degenerates to the original program. Now, we have the following new program, with
$\mathrm{(II)}\leq \mathrm{(I)}$. 
\begin{align*}
\mathrm{(II)}\triangleq \min_{\delta:\|\delta\|_1=c }
\min_{\one_r(\cdot)}
~~&
\frac1{b(2b)^d}
\int_{x\in \R^d}
\int_{r=\|x-\delta \|_1}^\infty 
\one_r(x)
e^{-\frac{r}{b}} dr dx\\
s.t. ~~&
\frac1{b(2b)^d}
\int_{x\in \R^d}
\int_{r=\|x \|_1}^\infty 
\one_r(x)
e^{-\frac{r}{b}} dr dx=\bar P
\end{align*}

Since both expressions are finite, we can change the integral, and get: 

\begin{align*}
\mathrm{(II)}= \min_{\delta:\|\delta\|_1=c }
\min_{\one_r(\cdot)}
~~&
\frac1{b(2b)^d}
\int_{r=0}^\infty 
e^{-\frac{r}{b}}\int_{x\in B_r(\delta)}
\one_r(x)
 dr dx\\
s.t. ~~&
\frac1{b(2b)^d}
\int_{r=0}^\infty 
e^{-\frac{r}{b}} 
\int_{x\in B_r(0)}
\one_r(x)
dr dx=\bar P
\end{align*}

For a given $\one_r(\cdot)$, 
define $\bar P_r\triangleq
\int_{x\in B_r(0)}
\one_r(x) dx
$, therefore we have 
\[
\int_{r=0}^\infty 
\frac{e^{-\frac{r}{b}} 
}{b(2b)^d}
\bar P_r dr= \bar P 
\]


Now, for a given $r$, given $\one_r(\cdot)$, and given $\delta$, below we show that we can always pick $\delta^*=(c,0,0,\cdots, 0)$ and $\one^*_r(\cdot)$, such that 
\begin{align*}
&\int_{x\in B_r(\delta)}
\one_r(x)
dr\geq \int_{x\in B_r(\delta^*)}
\one^*_r(x)
dr\\
s.t.& 
\int_{x\in B_r(0)}
\one_r(x) dx
=
\int_{x\in B_r(0)}
\one^*_r(x) dx=\bar P_r
\end{align*}

Denote $E_r\triangleq
\int_{x\in B_r(0)}
1 dx-\bar P_r
$. 
Pick $r'\geq 0$ such that 
$Vol(B_{r'}(\delta^*)\cap 
B_r(0))= E_r$, we may define $\one_r^*(x)=\one(x\in B_r(0)/(B_{r'}(\delta^*)\cap 
B_r(0)))$. By definition of $r'$, we know 
 $\int_{x \in B_r(0)}
\one^*_r(x) dx=\bar P_r$ holds. 

Below we show that 
\begin{equation}
\int_{x\in B_r(\delta)}
\one_r(x)
dr\geq \int_{x\in B_r(\delta^*)}
\one^*_r(x)
dr\label{eqn:replace_with_star}
\end{equation}

If $r'\geq r$, we know for any $x\in 
B_r(0)\cap B_r(\delta^*)$ or  any $x\not \in B_r(0)$, $\one^*_r(x)=0$. Therefore, $\int_{x\in B_r(\delta^*)}
\one^*_r(x)
dr=
\int_{x\in  B_r(\delta^*)\cap B_r(0)}
\one^*_r(x)
dr
+
\int_{x\in B_r(\delta^*)/B_r(0)}
\one^*_r(x)
dr
=0$, so (\ref{eqn:replace_with_star}) holds. 

If $r'<r$, we have:
\begin{align}
&\int_{x\in B_r(\delta^*)}
\one^*_r(x)
dr=
\int_{x\in  B_r(\delta^*)\cap B_r(0)}
\one^*_r(x)
dr
+
\int_{x\in B_r(\delta^*)/B_r(0)}
\one^*_r(x)
dr\nonumber\\
=&
\int_{x\in  B_r(\delta^*)\cap B_r(0)}
\one^*_r(x)
dr=
\mathrm{Vol}(B_r(\delta^*)\cap B_r(0))- 
\mathrm{Vol}
(B_{r'}(\delta^*)\cap B_r(0))\nonumber\\
=& \mathrm{Vol}(B_r(\delta^*)\cap B_r(0))-E_r \label{eqn:vol_1}
\end{align}

Similarly, we have 
\begin{align}
&\int_{x\in B_r(\delta)}
\one_r(x) dx=
\int_{x\in B_r(\delta)\cap B_r(0)}
\one_r(x) dx+
\int_{x\in B_r(\delta)/ 
 B_r(0)}
\one_r(x) dx\nonumber\\
\geq &
\int_{x\in B_r(\delta)\cap B_r(0)}
\one_r(x) dx=
\int_{x\in B_r(\delta)\cap B_r(0)}
1 dx-
\int_{x\in B_r(\delta)\cap B_r(0)}
(1-\one_r(x)) dx\nonumber\\
\geq &
\mathrm{Vol}(B_r(\delta)\cap B_r(0))-\int_{x\in B_r(0)}
(1-\one_r(x)) dx\nonumber
\\=&
\mathrm{Vol}(B_r(\delta)\cap B_r(0))-\left(\int_{x\in B_r(0)} 1 dx
-\int_{x\in B_r(0)}
\one_r(x) dx\right)\nonumber\\
=&\mathrm{Vol}(B_r(\delta)\cap B_r(0)) - E_r \label{eqn:vol_2}
\end{align}

The following Lemma says $\mathrm{Vol}(B_r(\delta^*)\cap B_r(0))\leq 
\mathrm{Vol}(B_r(\delta)\cap B_r(0))$. Combining (\ref{eqn:vol_1}) and (\ref{eqn:vol_2}), 
we have proved (\ref{eqn:replace_with_star}) for the case of $r'<r$. 

\begin{lem}
\label{lem:lower_bound_on_overlap}
For any $c, r, r'\geq 0$, any $\delta\in \R^d$ such that $\|\delta\|_1=c$, and $\delta^*=(c,0,0,\cdots, 0)\in \R^d$, we have
$\mathrm{Vol}(B_{r'}(\delta)\cap B_r(0))\leq 
\mathrm{Vol}(B_{r'}(\delta^*)\cap B_r(0))$. 
\end{lem}


\begin{proof}[Proof of Theorem \ref{lem:lower_bound_on_overlap}]
Without loss of generality, assume $r+r'\geq c\geq |r-r'|$, otherwise the intersection of the two balls will be empty, which means the claim is trivially true. 
Define $\xi\triangleq \frac{r+r'-c}{2}>0$.


Define $z\triangleq \frac{r -r' +c}{2c} \delta$. Notice that $r-r'+c \geq 0$, so 
\[
\|z\|_1 =\frac{r-r'+c}{2}= r-\xi 
\]

Therefore, 
for any point $z+x$, such that $\|x\|_1\leq \xi$, we know $\|z+x\|_1\leq 
\|z\|_1+\|x\|_1\leq r$. That is, 
$\gB_{1, \xi}(z)\in B_r(0)$.

On the other hand, since $\frac{r-r'+c}{2c}\leq 1$, we have
\[
\|z-\delta\|_1=
c-\frac{r-r'+c}{2}=
\frac{c-r+r'}{2}=r'-\xi
\]

That means, for any point $x+x$, such that $\|x\|_1\leq \xi$, we know $\|z+x- \delta \|_1\leq \|z-\delta \|_1+\|x\|_1\leq r'$. That is, 
$\gB_{1, \xi}(z)\in B_{r'}(\delta)$.

Combining two cases together, we have 
\begin{equation}
\gB_{1, \xi}(z)\in B_r(0)\cap B_{r'}(\delta)
\label{eqn:vol_any_delta}  
\end{equation}.

On the other hand, it is easy to see that 
\begin{equation}
\mathrm{Vol}(B_{r'}(\delta^*)\cap B_r(0))=
\mathrm{Vol}(\gB_{1, \xi}(z'))
\label{eqn:vol_star}    
\end{equation}
where $z'\triangleq (r-\xi, 0,0,\cdots, 0)$.
Combining (\ref{eqn:vol_any_delta}) and (\ref{eqn:vol_star}), we have proved our lemma. 
\end{proof}

Since we know (\ref{eqn:replace_with_star}) is true, we know that for any solution $\delta$, $\one_r(\cdot)$ for the program $\mathrm{(II)}$, we can always replace them with $\delta^*$, and our $\one^*_r(\cdot)$ to obtain at least equally small target value. More formally, we have  

\begin{align*}
&\frac1{b(2b)^d}
\int_{r=0}^\infty 
e^{-\frac{r}{b}}\int_{x\in B_r(\delta)}
\one_r(x)
 dx dr
\geq 
\frac1{b(2b)^d}
\int_{r=0}^\infty 
e^{-\frac{r}{b}}\int_{x\in B_r(\delta^*)}
\one_r^*(x)
 dx dr\\
\mathrm{and~~~~}&
\frac1{b(2b)^d}
\int_{r=0}^\infty 
e^{-\frac{r}{b}} 
\int_{x\in B_r(0)}
\one_r^*(x)
dx dr=\bar P
\end{align*}

That means, we can always use $\delta^*$ to solve the program $\mathrm{(II)}$. 
Now, fix $\delta^*$, the program $\mathrm{(II)}$ becomes:
\begin{align*}
\mathrm{(III)}\triangleq \min_{\one_r(\cdot)}
~~&
\frac1{b(2b)^d}
\int_{x\in \R^d}
\int_{r=\|x-\delta^* \|_1}^\infty 
\one_r(x)
e^{-\frac{r}{b}} dr dx\\
s.t. ~~&
\frac1{b(2b)^d}
\int_{x\in \R^d}
\int_{r=\|x \|_1}^\infty 
\one_r(x)
e^{-\frac{r}{b}} dr dx=\bar P
\end{align*}
For any given functions $\{\one_r(\cdot)\}_{r=0}^\infty$, we define \[\one'(x)\triangleq
\frac{\frac{1}{b(2b)^d}\int_{r=\|x \|_1}^\infty 
\one_r(x)
e^{-\frac{r}{b}} dr}{P(x)}\leq 
\frac{\frac{1}{b(2b)^d}\int_{r=\|x \|_1}^\infty 
e^{-\frac{r}{b}} dr
}{P(x)}=
1
\]

So we may rewrite the above program as:
\begin{align}
\mathrm{(III)}= \min_{\one'(\cdot)}
~~&
\int_{x\in \R^d}
\one'(x)P(x-\delta^*) dx\\
s.t. ~~&
\int_{x\in \R^d}
\one'(x)P(x) dx=\bar P
\label{eqn:one_constraint}
\end{align}

This is not the same program as $\mathrm{(I)}$, because $\one'(x)$ can take value from $[0,1]$ instead of $\{0,1\}$.

Below we will show, however, to minimize $\mathrm{(III)}$, it suffices to consider indicator functions, which means $\mathrm{(III)}$ and $\mathrm{(I)}$ have the same value.  

Define the likelihood function $\rho(x)\triangleq \frac{P(x)}{P(x-\delta^*)}\in [\rho_L, \rho_H]\triangleq [e^{-\frac{c}{b}}, e^{\frac{c}{b}}]$.
Define $L(t)\triangleq
\{
x: \rho(x)=t
\}
$, for $t\in [\rho_L, \rho_H]$. 
We have 
$\cup_{t=\rho_L}^{\rho_H} L(t)=\R^d$.
Therefore, we have
\begin{align}
& \int_{x\in \R^d } \one'(x) P(x-\delta^*) dx\\
 =&
 \int_{x\in \R^d } \one'(x)\frac{ P(x)}{\rho(x)} dx
 =
 \int_{t=\rho_L}^{\rho_H} \int_{x\in L(t) } \one'(x)\frac{ P(x)}{\rho(x)} dxdt\\
 =&
 \int_{t=\rho_L}^{\rho_H} 1/t\int_{x\in L(t) } \one'(x) P(x) dx dt \label{eqn:split_f_delta_eps}
 \end{align}

Let $\bar \rho$ be the maximum $\rho$ such that $
 \int_{t=\bar \rho }^{\rho_H } \int_{x\in L(t) } P(x) dx\geq  \bar P 
$. Notice that $\bar \rho$ always exists because  $ \int_{t=\rho_L}^{\rho_H } \int_{x\in L(t) } P(x) dx=1\geq \bar P $. 
Base on (\ref{eqn:split_f_delta_eps}), we have the following lower bound on $\mathrm{(III)}$. 
 
\begin{lem}\label{lem:likelihood}
Given any function $\one'(\cdot)\in \R^d\rightarrow [0,1]$  satisfying (\ref{eqn:one_constraint}),
$$\int_{x\in \R^d } \one'(x) P(x-\delta^*) dx\geq \int_{t=\bar \rho}^{ \rho_H } 1/t
\int_{x\in L(t) } P(x) dx$$ The equality holds when $\one'(x)$ is defined as 
\[ \one'(x) = \left\{ \begin{array}{ll}
        1 & \mbox{if $\rho(x)\geq \bar p$};\\
        0 & \mbox{if $\rho(x)< \bar p$}.\end{array} \right. \] 
\end{lem}

\begin{proof}
Define $\Delta(t)\triangleq 
\int_{x\in L(t) } \one\{t\geq \bar \rho\} P(x) dx 
- 
\int_{x\in L(t) } \one'(x) P(x) dx
$. From the definition of $\bar \rho$, we have
\[
\int_{t=\rho_L}^{\rho_H}\int_{x\in L(t) } \one\{t\geq \bar \rho\} P(x) dx dt
=\bar P 
=\int_{t=\rho_L}^{\rho_H}\int_{x\in L(t) } \one'(x) P(x) dxdt
\]

Therefore, $\int_{t=\rho_L}^{\rho_H} \Delta_f(t) =0$. Now, by (\ref{eqn:split_f_delta_eps}), we have
\begin{align}
& \int_{x\in \R^d } \one'(x) P(x-\delta^*) dx=   \int_{t=\rho_L}^{\rho_H} 1/t\int_{x\in L(t) } \one'(x) P(x) dxdt\\
=&
\int_{t=\rho_L}^{\rho_H} 1/t
\left(\int_{x\in L(t) }
\one\{t\geq \bar \rho\} P(x) dx -
\Delta_f(t)
\right)dt\\
=&
\int_{t=\bar \rho }^{\rho_H } 1/t
\int_{x\in L(t) } P(x) dxdt -
\int_{t=\rho_L}^{\rho_H} 
\frac{\Delta_f(t)}tdt
\label{eqn:minus_negative}
\end{align}

Notice that $\Delta_f(t)\geq 0$ for $t\geq \bar \rho$, and $\Delta_f(t)< 0$ for $t< \bar \rho$.
Therefore, we have 
\begin{equation}
\int_{t=\rho_L}^{\rho_H} 
\frac{\Delta_f(t)}t  dt\leq 
\int_{t=\rho_L}^{\bar \rho } 
\frac{\Delta_f(t)}{\bar \rho} dt
+
\int_{t=\bar \rho }^{\rho_H } 
\frac{\Delta_f(t)}{\bar \rho}dt
=0    
\label{eqn:sum_zero}
\end{equation}

Combining  (\ref{eqn:minus_negative}) and (\ref{eqn:sum_zero}), we have
$ \int_{x\in \R^d } \one'(x) P(x-\delta^*) dx\geq \int_{t=\bar \rho }^{\rho_H } 1/t
\int_{x\in L(t) } P(x) dx dt $.\end{proof}

Lemma \ref{lem:likelihood} tells us that to minimize program $\mathrm{(I)}$, it suffices to ``fill'' the indicator function according to the likelihood function $\rho(\cdot)$. For given $\delta^*$, $\rho$ has the following nice shape:

\[
\rho(x)= e^{\frac{-|x_1|+|x_1-c|}{b}}
\]

(TODO: calculation of $R$)



\section{Analysis}



Lemma \ref{lem:likelihood} tells us that for any given $\delta$, to minimize $\Pr(f(\delta+\eps)=c_A)$, we always pick the classifier that always predicts the wrong label for $\rho(x)<\bar \rho$. However, for different $\delta$, we have different lower bound in Lemma \ref{lem:likelihood}. Which $\delta$ gives the best lower bound? 

Below we show that for all $\delta$ with $\|\delta\|_1=R$, by setting $\delta=(R,0,0,\cdots, 0)$ we get the smaller lower bound from Lemma \ref{lem:likelihood}. 

Denote the  sphere of the $\ell_1$ ball centered at $x$ with radius $r$ as $S_{r}(x)\triangleq \{x': \|x-x'\|_1 = r\}$. Therefore, we can rewrite $\Pr(f(\eps)=c_A)$ as the integral of infinitely many stacked spheres:

\begin{align}
 \bar P= \Pr(f(\eps)=c_A)
 &=\int_{r=0}^\infty 
\int_{x'\in S_r(0)} \one(x') P(x') dx' dr
\\&=\frac1{(2b)^d}\int_{r=0}^\infty 
e^{- \frac{r}{b}}
\int_{x'\in S_r(0)} \one(x')  dx' dr
\end{align}

 Let $\bar \rho\triangleq \argmax_\rho 
 \int_{t=\bar \rho }^{\rho_H } \int_{x'\in L(t) } P(x') dx'\geq  \bar P 
$. Define likelihood ratio function $\rho(x')\triangleq \frac{P(x')}{P(x'-\delta)}
= e^{- \frac{\|x'\|_1- \|x'-\delta\|_1}{b}}
\in [e^{-\frac{\|\delta\|_1 }{b}}, e^{\frac{\|\delta\|_1 }{b}}]\triangleq
[\rho_L, \rho_H]$.

Using the notion of $S_r(x)$, we can rewrite the lower bound of $\Pr(f(\delta+\eps)=c_A)$ as: 
\begin{align*}
&    \Pr(f(\delta+\eps)=c_A)\geq \int_{t=\bar \rho}^{ \rho_H } 1/t
\int_{x'\in L(t) } P(x') dx' dt\\
=&
\int_{t=\bar \rho}^{ \rho_H } 1/t
\int_{r=0}^{\infty}
\int_{x'\in S_r(0) \cap L(t) } P(x') dx'drdt\\
=&
\int_{t=\bar \rho}^{ \rho_H } 1/t
\int_{r=0}^{\infty}
\int_{x'\in S_r(0) \cap \left \{
x': \frac{P(x')}{P(x'-\delta)}=t
\right \} } P(x') dx'drdt\\
=&
\frac{1}{(2b)^d}
\int_{t=\bar \rho}^{ \rho_H } 1/t
\int_{r=0}^{\infty}
\int_{x'\in S_r(0) \cap \left \{
x': e^{-\frac{r-\|x'-\delta\|_1}{b}}=t
\right \} }  e^{-\frac{r}{b}} dx'drdt\\
=&
\frac{1}{(2b)^d}
\int_{t=\bar \rho}^{ \rho_H } 1/t
\int_{r=0}^{\infty}e^{-\frac{r}{b}}
\mathrm{Vol}\left (S_r(0) \cap \left \{
x': e^{-\frac{r-\|x'-\delta\|_1}{b}}=t
\right \} \right )drdt\\
\end{align*}


Let $r_2\triangleq r+b\log t\leq r+\|\delta\|_1$. 
Without loss of generality, we may assume 
$r_2\geq 0$, otherwise 
$
\left \{
x': e^{-\frac{r-\|x'-\delta\|_1}{b}}=t
\right \}=\varnothing$. 
Now, we have
$\left \{
x': e^{-\frac{r-\|x'-\delta\|_1}{b}}=t
\right \}= S_{r_2}(\delta)$.
To get the lower bound of $\Pr(f(\delta+\eps)=c_A)$, we need to understand the term $\mathrm{Vol}\left (S_r(0) \cap S_{r_2}(\delta) \right )$. We first introduce the following notion. 

\begin{definition}
We say $\delta\in \R^d$ is concentrated, if there exists $i\in [d]$ such that $\delta_i=\|\delta\|_1$.
\end{definition}
For example, $(R,0,0,\cdots, 0)$ is concentrated, but $(R/2, R/2, 0,0, \cdots, 0)$ is not.

\begin{lem}
\label{lem:lower_bound_on_overlap_sphere}
Given constant $c,r_1,r_2>0$, 
for any $\delta, \delta'\in \R^d$ such that $\|\delta\|_1=\|\delta'\|_1=c$ and 
$\delta'$ is concentrated, and
for any $t\in (\rho_L, \rho_H)$, 
we have 
$\mathrm{Vol}\left (S_{r_1}(0) \cap S_{r_2}(\delta)  \right )
\geq 
\mathrm{Vol}\left (S_r(0) \cap S_{r_2}(\delta') \right )$.
\end{lem}

For any $\delta$ with  $\|\delta\|_1=c$, we assume $r_1+r_2 \geq c\geq |r_1-r_2|$, otherwise these two spheres do not overlap, which means $S_{r_1}(0)\cap S_{r_2}(\delta)=\varnothing$. 

Denote $\xi\triangleq \frac{r_1+r_2-c}{2}\geq 0$. Notice that 
\begin{equation}
\label{eqn:xi_ordering}
r_1-\xi=\frac{r_1-r_2+c}{2} >0
\end{equation}
\begin{equation}
\label{eqn:xi_ordering_2}
r_2-\xi=
\frac{r_2+c-r_1}{2}>0
\end{equation}

\begin{proof}[Proof of Theorem \ref{lem:lower_bound_on_overlap_sphere}]
Without loss of generality, we may assume $\delta'=(c, 0,0,\cdots, 0)$. 


Since $\delta_1$ is concentrated, 
for every $x\in S_r(0) \cap S_{r_2}(\delta')$, we have
\[\left\{ \begin{array}{ll}
        \sum_i |x_i| = r_1;\\
        |x_1-c|+\sum_{i>1} |x_i|= r_2.\end{array} \right. \] 

That gives $|x_1|-|x_1-c|=r_1-r_2$. 
Now we can do case analysis. If $x_1<0$, this equality gives us $0>-c=r_1-r_2>0$, which is a contradiction. If $0\leq x_1\leq c$, we have $x_1=\frac{r_1-r_2+c}{2}=r_1-\xi $. 
If $x_1>\delta_1$, we have $c=r_1-r_2$, which contradicts our assumption that $r_2>r_1-c$. Therefore, the only possibility is $0\leq x_1\leq c$ and $x_1=r_1-\xi\geq 0$.
    
Therefore, we have $\sum_{i>1} |x_i| = r_1 -r_1+\xi = \xi $. That means, 
$S_r(0) \cap S_{r_2}(\delta')$ can be seen as a $d-1$ dimension $\ell_1$ ball with radius $\xi$ for $x_2, \cdots, x_d$. 

Now we use induction on dimension $d$ to show $\mathrm{Vol}\left (S_{r_1}(0) \cap S_{r_2}(\delta)  \right )
\geq 
\mathrm{Vol}\left (S_{r_1}(0) \cap S_{r_2}(\delta') \right )$. Due to symmetry, below we assume $\delta_i\geq 0$ for all $i\in [d]$. 

We assume the following is true: $
\xi=\frac{r_1+r_2-\|\delta\|_1}{2},
r_1\geq \xi, r_2\geq \xi$. 

\textbf{Base case $d=2$}:
Trivially true. 

\textbf{$d>2$}:
Assume $d-1$ dimension case is true, and we consider the dimension $d$ case. 

We will show that for any $(x_2, \cdots, x_d)\in S_{\xi}^{d-1}(0)$, we could find another point in 
$S_{r_2}(\delta')$ by a linear shift. 
We will do a case analysis. Notice that $|x_2|\leq \xi$.

\begin{itemize}
\item If $r_1\geq \xi+\delta_1$. In this case, if $x_2\geq 0$, we pick $y_1=\delta_1+x_2$. Now, to find solution $(y_2, \cdots, y_d)\in \R^{d-1}$, it suffices to satisfy the following for $d-1$ dimensional case: 
\[\left\{ \begin{array}{ll}
r_1'\leftarrow r_1-x_2-\delta_1;\\
r_2'\leftarrow r_2-x_2;\\
\delta'\leftarrow (\delta_2, \cdots, \delta_d);\\
\xi'\leftarrow \frac{r_1'+r_2'-\|\delta'\|_1}{2}=\frac{r_1+r_2-2x_2-\delta_1-\|\delta\|_1+\delta_1}{2}=\xi-x_2.\end{array} \right. \] 

therefore, we have $r_1'=r_1-x_2-\delta_1\geq \xi+\delta_1-x_2-\delta_1=\xi-x_2=\xi'$, and $r_2'\geq \xi-x_2=\xi'$. Therefore, we reduce the problem into the $d-1$ dimensional case, and we know that the volume is at least the ball. So $x_2\geq 0$ case is covered. 

If $x_2<0$, we can do another case analysis:
\begin{enumerate}
    \item If $r_2\geq \xi+\delta_1$. In this case, we pick $y_1=x_2<0$.  Now, to find solution $(y_2, \cdots, y_d)\in \R^{d-1}$, it suffices to satisfy the following for $d-1$ dimensional case: 
\[\left\{ \begin{array}{ll}
r_1'\leftarrow r_1-|x_2|;\\
r_2'\leftarrow r_2-\delta_1- |x_2|;\\
\delta'\leftarrow (\delta_2, \cdots, \delta_d);\\
\xi'\leftarrow \frac{r_1'+r_2'-\|\delta'\|_1}{2}=\frac{r_1+r_2-\delta_1-\|\delta\|_1+\delta_1-2|x_2|}{2}=\xi-|x_2|.\end{array} \right. \] 
therefore, we have $r_1'=r_1-|x_2|\geq \xi-|x_2|=\xi'$, and $r_2'\geq \xi+\delta_1-\delta_1-|x_2|= \xi'$. Therefore, we reduce the problem into the $d-1$ dimensional case, and we know that the volume is at least the ball. 

\item If $r_2< \xi+\delta_1$.
 In this case, we pick $y_1=
 \delta_1+\xi -r_2$, since $r_2>\xi$, we have $\delta_1>y_1>0$. 
Notice that $r_1+r_2-\xi -\delta_1\geq 
r_1+r_2-\xi -\|\delta\|_1
=\xi $.
Now, to find solution $(y_2, \cdots, y_d)\in \R^{d-1}$, it suffices to satisfy the following for $d-1$ dimensional case: 
\[\left\{ \begin{array}{ll}
r_1'\leftarrow r_1-(\delta_1+\xi-r_2)=
r_1+r_2-\xi -\delta_1
\geq \xi 
;\\
r_2'\leftarrow r_2-(\delta_1-(\delta_1+\xi-r_2))\geq \xi;\\
\delta'\leftarrow (\delta_2, \cdots, \delta_d);\\
\xi'\leftarrow \frac{r_1'+r_2'-\|\delta'\|_1}{2}=\frac{r_1+r_2-\delta_1-\|\delta\|_1+\delta_1}{2}=\xi.\end{array} \right. \] 

This case is special, as for the $d-1$ dimensional problem, $r_2'=\xi$, therefore $r_1'=
2\xi +\|\delta'\|_1-r_2'=
\|\delta'\|_1+\xi$. 


therefore, we have $r_1'=r_1-x_2-\delta_1\geq \xi+\delta_1-x_2-\delta_1=\xi-x_2=\xi'$, and $r_2'\geq \xi-x_2=\xi'$. Therefore, we reduce the problem into the $d-1$ dimensional case, and we know that the volume is at least the ball. So $x_2\geq 0$ case is covered. 
\end{enumerate}
So $x_2< 0$ case is also covered.



\item If $r_1<\xi+\delta_1$.
\end{itemize}

Now, for any $\delta$ such that $\|\delta\|_1=c$, define $y= \frac{r_1 -r_2 +c}{2c} \delta$. Based on (\ref{eqn:xi_ordering})
\[
\|y\|_1 =\frac{r_1-r_2 +c}{2}= r_1 -\xi
\]

For any 
$x\in S_r(0) \cap S_{r_2}(\delta')$, we define $x'$ as follows:
\[x'_i=\left\{ \begin{array}{ll}
        \xi-r_2+\delta_1& i=1;\\
        x_i +\delta_i;& i>1.\end{array} \right. \] 

Therefore, based on (\ref{eqn:xi_ordering_2})
\[
\|x'-\delta\|_1=|r_2-\xi|+ \sum_{i>1} |x_i|=r_2
\]


On the other hand, we have 
\[
\|x'\|_1= 
\sum_{i>1} |x_i +\delta_i|=
\sum_{i>1} |x_i| + |\delta_i| =
\xi+ c + \xi-r_2 =r_1
\]

Therefore, 
for any point $\vx+z$, such that $\|z\|_1\leq \xi_3$, we know $\|\vx+z\|_1\leq 
\|\vx\|_1+\|z\|_1\leq \xi_1$. That is, 
$\gB_{1, \xi_3}(\vx)\in A$.

On the other hand, since $\frac{\xi_1 -\xi_2 +\|\delta\|_1}{2\|\delta\|_1}\leq 1$, we have
\[
\|\vx-\delta\|_1=
\|\delta\|_1-\frac{\xi_1 -\xi_2 +\|\delta\|_1}{2}=
\frac{\|\delta\|_1-\xi_1 +\xi_2}{2}=\xi_2-\xi_3
\]

That means, for any point $\vx+z$, such that $\|z\|_1\leq \xi_3$, we know $\|\vx+z- \delta \|_1\leq \|\vx-\delta \|_1+\|z\|_1\leq \xi_2$. That is, 
$\gB_{1, \xi_3}(\vx)\in B$.

Combining two cases together, we have $\gB_{1, \xi_3}(\vx)\in A\cap B$.

\end{proof}

Based on this, we have the following lemma: 
\begin{lem}
$\bar \rho $ gets its maximum when $\delta=(R,0,0,\cdots, 0)$. 
\end{lem}


We want to maximize the following integral. 
\begin{align}
\int_{t=\rho_L}^{ \bar \rho } 1/t
\int_{r=0}^{\infty}e^{-\frac{r}{b}}
\mathrm{Vol}\left (S_r(0) \cap S_{r'}(\delta) \right )drdt
\end{align}

We have the following lemma: 
\begin{lem}
\[
\int_{t=\rho_L}^{ \bar \rho  } 1/t
\mathrm{Vol}\left (S_r(0) \cap S_{r_2}(\delta)\right )dt
\]
gets its maximum when $\delta$ is concentrated. 
\end{lem}

\begin{proof}
First, we know that the total probability that we put $0$ is fixed. It is equal to $1-\bar P$. 

On the other hand, we know that the score for $P(x-\delta)$ is controlled by $1/t$, which means, the mass of $0$ put on level $t$ gets scaled by $1/t$ in the final score. 

Notice that the previous lemma says the intersection of $t>\rho_L$ is minimized when $\delta$ is concentrated. On the other hand, it is easy to see that on the level of $t=\rho_L$, the intersection when $\delta$ is concentrated is maximized. Therefore, for concentrated $\delta$, it gets more ``high score'' regions, and less ``low score'' regions. That tells that score is maximized here. 
\end{proof}

Since the score of $P(x-\delta)$ on $0$ is maximized, therefore the score of $P(x-\delta)$ on $1$ is minimized as their sum is $1$. 


\section{The Laplacian Case}

\begin{lem}
$\forall \vx \in \sR^d, \xi_1, \xi_2, v > 0$,   
\begin{align}
    \{-v \ve^i, v \ve^i\}_{i=1}^d \subseteq \argmin_{\delta \in \sR^d: \|\delta\|_1 \leq v} \text{Vol}(\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta)).
\end{align}
\end{lem}


\begin{proof}
New version

We first make the following trivial observation:
\begin{itemize}
    \item The minimizers lie in the sphere $\delta^* \in \sR^d: \|\delta\|_1 = v$.
    \item Due to the symmetry, the case when $\delta_k > 0, \forall k \in [d]$ generalizes to all the other cases.
    \item Due to the symmetry, the volume is the same across the set $\{-v \ve^i, v \ve^i\}_{i=1}^d$.
\end{itemize}
$\forall \delta \in \sR^d$ such that $\|\delta\|_1 = v$ and $\delta_k > 0, \forall k \in [d]$, we set 
\begin{align}
    i := \argmax_{k \in [d]} |\delta_k|,
\end{align}
where $i$ can be an arbitrary maximizer when multiple ones exist. We set $\delta^* = v \ve^i$, and we have
% \begin{align}
%     \begin{cases}
%         \delta^*_i = v, &\\
%         \delta^*_k = 0,& \forall k \in [d], k \neq i.
%     \end{cases}
% \end{align}
\begin{align}
    & \forall \vz \in \gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta^*), \vz + \delta - \delta^* \in \gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta) \label{eq:assump} \\
    \implies & \text{Vol}(\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta^*)) \leq \text{Vol}(\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta)).
\end{align}

Case 1 $\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta^*) = \{\}$: the conclusion is trivial.

Case 2 $\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta^*) \neq \{\}$: it implies $v \leq \xi_1 + \xi_2$. To simplify notation, we denote:
\begin{enumerate}
    \item $A := \gB_{1, \xi_1}(\vx) = \{\vz \in \sR^d: \|\vx - \vz \|_1 \leq \xi_1\}$.
    \item $B := \gB_{1, \xi_2}(\vx + \delta) = \{\vz \in \sR^d: \|\vx + \delta - \vz \|_1 \leq \xi_2\}$.
    \item $\bar B := \gB_{1, \xi_2}(\vx + \delta^*) = \{\vz \in \sR^d: \|\vx + \delta^* - \vz \|_1 \leq \xi_2\}$.
\end{enumerate}

Since $A \cap B$ is convex, we only have to show that the extreme points of $A \cap \bar B + \delta - \delta^* \subseteq A \cap B$ in order to prove Eq.~(\ref{eq:assump}). We first observe that $A \cap \bar B$ is an $\ell_1$ ball with radius $\xi_3 := 0.5(\xi_1 + \xi_2 - v)$:
\begin{align}
    A \cap \bar B = \{ \vz \in \sR^d: \| ( \vx + (\xi_1 - \xi_3)\ve^i ) - \vz \|_1 \leq \xi_3\}.
\end{align}
As a result, the set of the extreme points is 
\begin{align}
    C := \{\vx + (\xi_1 - \xi_3)\ve^i + \xi_3\ve^k, \vx + (\xi_1 - \xi_3)\ve^i - \xi_3\ve^k\}_{k=1}^d.
\end{align}
First, we show $C + \delta - \delta^* \subseteq A$ by
\begin{align}
    & \forall \vz \in C + \delta - \delta^*, \| \vz - \vx \|_1 \leq \|\vx + (\xi_1 - \xi_3)\ve^i + \delta - \delta^* - \vx \|_1 + \xi_3 \\
    & = | \xi_1 - \xi_3 + \delta_i - v | + \sum_{k \in [d]: k \neq i} \delta^k + \xi_3 = \xi_1
\end{align}
where we use triangle inequality, and $\xi_1 - \xi_3 + \delta_i - v \geq 0$ is due to (currently wrong)
\begin{align}
    \xi_1 - \xi_3 + \delta_i - v = 0.5 \xi_1 - 0.5 \xi_2 - 0.5 v + \delta_i \geq 0.5 \xi_1 - 0.5 \xi_2 - 0.5 v
\end{align}

Second, we show $C + \delta - \delta^* \subseteq B$ by
\begin{align}
    & \forall \vz \in C + \delta - \delta^*, \|\vz - \vx - \delta\|_1 \leq \|\vx + (\xi_1 - \xi_3)\ve^i + \delta - \delta^* - \vx - \delta\|_1 + \xi_3 \\
    & = | \xi_1 - \xi_3 - v | + \xi_3 = v + 2\xi_3 - \xi_1 = \xi_2.
\end{align}

\end{proof}

% \begin{proof}
% We first make the following trivial observation:
% \begin{itemize}
%     \item The minimizers lie in the sphere $\delta^* \in \sR^d: \|\delta\|_1 = v$.
%     \item Due to the symmetry, the case when $\delta_k > 0, \forall k \in [d]$ generalizes to all the other cases.
%     \item Due to the symmetry, the volume is the same across the set $\{-v \ve^i, v \ve^i\}_{i=1}^d$.
% \end{itemize}
% $\forall \delta \in \sR^d$ such that $\|\delta\|_1 = v$ and $\delta_k > 0, \forall k \in [d]$, we set 
% \begin{align}
%     i := \argmax_{k \in [d]} |\delta_k|,
% \end{align}
% where $i$ can be an arbitrary maximizer when multiple ones exist. We set $\delta^* = v \ve^i$, and we have
% % \begin{align}
% %     \begin{cases}
% %         \delta^*_i = v, &\\
% %         \delta^*_k = 0,& \forall k \in [d], k \neq i.
% %     \end{cases}
% % \end{align}
% \begin{align}
%     & \forall \vz \in \gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta^*), \vz + \delta - \delta^* \in \gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta) \label{eq:assump} \\
%     \implies & \text{Vol}(\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta^*)) \leq \text{Vol}(\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta)).
% \end{align}

% Case 1 $\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta^*) = \{\}$: the conclusion is trivial.

% Case 2 $\gB_{1, \xi_1}(\vx) \cap \gB_{1, \xi_2}(\vx + \delta^*) \neq \{\}$: it implies $v \leq \xi_1 + \xi_2$. To simplify notation, we denote:
% \begin{enumerate}
%     \item $A := \gB_{1, \xi_1}(\vx) = \{\vz \in \sR^d: \|\vx - \vz \|_1 \leq \xi_1\}$.
%     \item $B := \gB_{1, \xi_2}(\vx + \delta) = \{\vz \in \sR^d: \|\vx + \delta - \vz \|_1 \leq \xi_2\}$.
%     \item $\bar B := \gB_{1, \xi_2}(\vx + \delta^*) = \{\vz \in \sR^d: \|\vx + \delta^* - \vz \|_1 \leq \xi_2\}$.
% \end{enumerate}

% Since $A \cap B$ is convex, we only have to show that the extreme points of $A \cap \bar B + \delta - \delta^* \subseteq A \cap B$ in order to prove Eq.~(\ref{eq:assump}). We first observe that $A \cap \bar B$ is an $\ell_1$ ball with radius $\xi_3 := 0.5(\xi_1 + \xi_2 - v)$:
% \begin{align}
%     A \cap \bar B = \{ \vz \in \sR^d: \| ( \vx + (\xi_1 - \xi_3)\ve^i ) - \vz \|_1 \leq \xi_3\}.
% \end{align}
% As a result, the set of the extreme points is 
% \begin{align}
%     C := \{\vx + (\xi_1 - \xi_3)\ve^i + \xi_3\ve^k, \vx + (\xi_1 - \xi_3)\ve^i - \xi_3\ve^k\}_{k=1}^d.
% \end{align}
% First, we show $C + \delta - \delta^* \subseteq A$ by
% \begin{align}
%     & \forall \vz \in C + \delta - \delta^*, \| \vz - \vx \|_1 \leq \|\vx + (\xi_1 - \xi_3)\ve^i + \delta - \delta^* - \vx \|_1 + \xi_3 \\
%     & = | \xi_1 - \xi_3 + \delta_i - v | + \sum_{k \in [d]: k \neq i} \delta^k + \xi_3 = \xi_1
% \end{align}
% where we use triangle inequality, and $\xi_1 - \xi_3 + \delta_i - v \geq 0$ is due to (currently wrong)
% \begin{align}
%     \xi_1 - \xi_3 + \delta_i - v = 0.5 \xi_1 - 0.5 \xi_2 - 0.5 v + \delta_i \geq 0.5 \xi_1 - 0.5 \xi_2 - 0.5 v
% \end{align}

% Second, we show $C + \delta - \delta^* \subseteq B$ by
% \begin{align}
%     & \forall \vz \in C + \delta - \delta^*, \|\vz - \vx - \delta\|_1 \leq \|\vx + (\xi_1 - \xi_3)\ve^i + \delta - \delta^* - \vx - \delta\|_1 + \xi_3 \\
%     & = | \xi_1 - \xi_3 - v | + \xi_3 = v + 2\xi_3 - \xi_1 = \xi_2.
% \end{align}

% \end{proof}

\section{Method for 0319 meeting}

\begin{enumerate}
    \item $\ell_1$-norm certificate on uniform distributions.
    \item $\ell_1$-norm certificate on mixture of uniform distributions.
    \item Learning $\sigma$ in the Gaussian perturbations.
    \item Hinge-loss does not work. 
    \item Modeling local landscape.
\end{enumerate}

\header{Notations}
\begin{enumerate}
    \item We have noise $\epsilon \sim \mathcal{D}$ according to a distribution $\mathcal{D}$.
    \item $\mathcal{F}$ is the set of measurable functions w.r.t. $\mathcal{D}$.
    \item The label class is denoted as $c \in \gC$. 
\end{enumerate}

\begin{lem}
$\forall \vx \in \sR^d, f \in \mathcal{F}$, with $p := \sP_{\epsilon}(f(\vx + \epsilon) = c) > 0.5$, and we define
\begin{align}
    R(\vx, p) & = \sup \| \delta \|_q \\
    s.t. & \inf_{\bar{f} \in \mathcal{F}: \sP_{\epsilon}(\bar{f}(\vx + \epsilon) = c) = p} \sP_{\epsilon}(\bar{f}(\vx + \delta + \epsilon) = c) > 0.5.
\end{align}
Then $\sP_{\epsilon}(\bar{f}(\vx + \delta + \epsilon) = c) > 0.5$ whenever $\|\delta\|_q < R(\vx, p)$, and the bound is tight.  
\end{lem}

\begin{proof}
If $\| \delta \|_q < R(\vx, p)$, we know 
\begin{align}
    \sP_{\epsilon}(f(\vx + \delta + \epsilon) = c) \geq \inf_{\bar{f} \in \mathcal{F}: \sP_{\epsilon}(\bar{f}(\vx + \epsilon)) = p} \sP_{\epsilon}(\bar{f}(\vx + \delta + \epsilon) = c) > 0.5.
\end{align}
If $\| \delta \|_q > R(\vx, p)$, $\exists \bar{\delta} \in \sR^D: \| \delta \|_q > \|\bar{\delta}\|_q > R(\vx, p)$ s.t.
\begin{align}
    & \inf_{\bar{f} \in \mathcal{F}: \sP_{\epsilon}(\bar{f}(\vx + \epsilon) = c) = p} \sP_{\epsilon}(\bar{f}(\vx + \bar{\delta} + \epsilon) = c) \leq 0.5 \text{ and } \exists \bar{f} \in \gF: \sP_{\epsilon}(\bar{f}(\vx + \delta + \epsilon) = c) \leq 0.5;
\end{align}
otherwise, it will lead to contradiction. 
\end{proof}

\begin{prop}
If $q = \infty$, $\gD = \text{Unif}([-\alpha, \alpha]^d)$, $R(\vx, p) = {2\alpha - } 2\alpha(1.5 - p)^{1/d}$.
\end{prop}

\begin{proof}
$\forall \delta \in \sR^d: \|\delta\|_\infty > 0$,
\begin{align}
    \inf_{\bar{f} \in \mathcal{F}: \sP_{\epsilon}(\bar{f}(\vx + \epsilon) = c) = p} \sP_{\epsilon}(\bar{f}(\vx + \delta + \epsilon) = c) = p - (1 - \frac{(2\alpha - \|\delta\|_\infty)^d}{(2\alpha)^d}),
\end{align}
which is larger than $0.5$ iff
\begin{align}
    & \frac{(2\alpha - \|\delta\|_\infty)^d}{(2\alpha)^d} > 1.5 - p \\
    \iff & {2\alpha - \|\delta\|_\infty} > 2\alpha(1.5 - p)^{1/d} \\
    \iff & {2\alpha - } 2\alpha(1.5 - p)^{1/d} > \|\delta\|_\infty.
\end{align}
\end{proof}


\begin{prop}
If $q = 1$, $\gD = \text{Unif}([-\alpha, \alpha]^d)$, $R(\vx, p) = {2p \alpha - } \alpha$.
\end{prop}

\begin{proof}
$\forall v > 0$, to find the infimum of $\delta$
\begin{align}
    \inf_{\delta: \|\delta\|_1 \leq v} \inf_{\bar{f} \in \mathcal{F}: \sP_{\epsilon}(\bar{f}(\vx + \epsilon) = c) = p} \sP_{\epsilon}(\bar{f}(\vx + \delta + \epsilon) = c) \label{eq:l1}
\end{align}
is the same as finding the following minimizer  
\begin{align}
    \argmin_{\delta\geq 0: \|\delta \|_1 = v} \prod_{i=1}^d (2\alpha - \delta_i).
\end{align}
Since $\forall i, j \in [d], i\neq j$, we know
\begin{align}
    (2\alpha - \delta_i)(2\alpha - \delta_j) = 4\alpha^2 - (\delta_i + \delta_j) + \delta_i \delta_j \geq 4\alpha^2 - (\delta_i + \delta_j).
\end{align}
Hence, we know $\delta_1 = 1, \delta_i = 0, \forall i \neq 1$ is a minimizer and minimizes Eq. (\ref{eq:l1}) for a fixed $\|\delta\|_1$. As a result, we know 
\begin{align}
    & \sup v, s.t.\text{   } \inf_{\delta: \|\delta\|_1 \leq v} \inf_{\bar{f} \in \mathcal{F}: \sP_{\epsilon}(\bar{f}(\vx + \epsilon) = c) = p} \sP_{\epsilon}(\bar{f}(\vx + \delta + \epsilon) = c) > 0.5 \\
    = & \sup v, s.t.\text{   } p - (1 - \frac{(2\alpha)^{d-1}(2\alpha - v)}{(2\alpha)^{d}}) > 0.5 \\
    = & \sup v, s.t.\text{   } p - (1 - \frac{(2\alpha)^{d-1}(2\alpha - v)}{(2\alpha)^{d}}) > 0.5 \\
    = & 2p \alpha - \alpha
\end{align}
\end{proof}

\section{Multiple high dimensional cubes}
We consider the following scenario: we have $k$ $l_\infty$ balls (i.e., high dimensional cubes), each with radius $r_k$, satisfying $r_k>2 r_{k-1}$. 

Assume that we are now at the input $x$. 
We would like to find a distribution over these cubes, denoted as $\{p_i\}_{i=1}^k$, such that they could give us the optimal certificate. 
Denote the resulting probability distribution as $H$, 
and denote $\bar P=\Pr_{\eps \sim H} (f(x+\eps)=A)$. That is, the probability that $f$ correctly classifies $x+\eps$ as class $A$, under the perturbation $\eps\sim  H$. 

Using the overlapping argument, we are trying to find the optimal distribution such that we could have the largest  $r_0$ s.t. $\|\delta \|_\infty\leq r_0$, and after the shift $\delta$, the overlapping measure is larger than $1.5-\bar P$. 

It seems that the following lemma is true:
\begin{lem}
In the worst case that minimizes the overlapping measure, we always have $|\delta_i|=r_0$ for every $i\in [d]$. 
\end{lem}
\begin{proof}
The overlapping measure is monotone as $|\delta_i|$ goes toward $r_0$. 
\end{proof}

If Lemma 1 holds, we know that $|\delta_i|=r_0$ for every $i$. By symmetry, WLOG we may set $\delta_i=r_0$. 

Therefore, by symmetry, the overlapping region in $d$ dimensional space can be well characterized in $1$ dimension. We also have the following lemma: 

\begin{lem}\label{lem:3k}
If $r_k>2r_{k-1}$, we have at most $3k$ regions with different likelihood ratios.
\end{lem}
\begin{proof}
The two distributions have the same set of cubes. Denote the smallest pair of cubes that are overlapped with each other as $i$. We have the following claim: for every $j>i$, cube $j$ can only overlap with its corresponding pair. 

Therefore, we can do simple counting and get $3k$ regions.  
\end{proof}

\textbf{Remark}. Lemma \ref{lem:3k} is not particularly important, because a trivial counting will give us $k^2$ regions, which is still affordable for reasonable $k$. 

Notice that we could use stack to compute the volume in each region efficiently by a linear scan, for a given $r_0$. 

With given $\{p_i\}$, we can also determine the probability of each region, under the two distributions. Therefore, we can sort them, and calculate the final overlapping measure using the expression of $\{p_i\}$. We hope that the overlapping measure is larger than $1.5-\bar P$. To get the gradient of $\{p_i\}$, we may simply maximize the overlapping measure, such that it becomes larger than $1.5-\bar P$. That means, we could aim for a larger $r_0$. After updating $\{p_i\}$, we will use binary search to update $r_0$, and keep doing it until convergence. 





\section{Method for 0305 meeting}

\begin{prop}
(CMU - 2) Let $f: \mathbb{R}^d \to \mathcal{Y}$ be any deterministic or random function, and let $\epsilon \sim N(0, \sigma^2 I)$. Let 
\begin{align}
    & g(x) := \argmax_{c \in \mathcal{Y}} \mathbb{P}(f(x + \epsilon) = c)
\end{align}
Suppose $\underline{p_A} > 0.5$ are such that:
\begin{equation}
    \mathbb{P}(f(x+\epsilon) = c_A) \geq \underline{p_A} \geq (1 - \underline{p_A}) \geq \max_{c \neq c_A} \mathbb{P}(f(x+\epsilon) = c)
\end{equation}
Then $g(x) = g(x + \delta)$ whenever $\|\delta\|_2 < R$, where
\begin{equation}
    R := \frac{\sigma}{2} (\Phi^{-1}(\underline{p_A}) - \Phi^{-1}(1 - \underline{p_A})) = \sigma \Phi^{-1}(\underline{p_A}).
\end{equation}
\end{prop}
We may assume a $\delta$-margin is a given, given radius that we want to enforce robustness, and $\sigma$ is a \emph{variable}. The loss at testing time is thus:
\begin{equation}
    \frac{1}{n} \sum_{i \in [n]} \mathbb{I} (\sigma \Phi^{-1}(\mathbb{P}(f(x_i + \epsilon) = y_i) ) > \delta)
\end{equation}

\subsection{Optimizing the certified radius}

For simplicity, we first assume that the label $y_i$ is known, then we can optimize the certified radius w.r.t. $\sigma$ as:
\begin{align}
    & \max_{\sigma > 0} \sigma \Phi^{-1}(\mathbb{E}_{\epsilon\sim \mathcal{N}(0, \sigma^2 I)}[P_\theta(y_i | x_i + \epsilon)]  ) \\
    = & \max_{\sigma > 0} \sigma \Phi^{-1}(\mathbb{E}_{\epsilon\sim \mathcal{N}(0, \bar{\sigma}^2 I)}[\frac{\prod_{k \in [D]} \mathcal{N}(\epsilon_k ; 0, \sigma^2)}{\prod_{k \in [D]} \mathcal{N}(\epsilon_k ; 0, \bar{\sigma}^2)}  P_\theta(y_i | x_i + \epsilon)]  ) \\
    = & \max_{\sigma > 0} \sigma \Phi^{-1}(\mathbb{E}_{\epsilon\sim \mathcal{N}(0, \bar{\sigma}^2 I)}[\frac
    {\prod_{k \in [D]} \bar{\sigma} \exp(-\epsilon_k^2 / 2\sigma^2))}
    {\prod_{k \in [D]} \sigma \exp(-\epsilon_k^2 / 2\bar{\sigma}^2)) }  P_\theta(y_i | x_i + \epsilon)]  ) 
\end{align}
Since the quantile function $\Phi^{-1}$ is not differentiable, we use an approximation to the quantile function\footnote{http://m-hikari.com/ams/ams-2014/ams-85-88-2014/epureAMS85-88-2014.pdf}:
\begin{align}
    & \hat{\Phi}^{-1}(p) := \frac{10}{\log 41} \log (1 -  \frac{\log ((-\log p) /\log 2)}{\log 22},  \forall \infty > p \geq 1/2,\\
    & \hat{\Phi}^{-1}(p) := - \hat{\Phi}^{-1}(1 - p), \forall -\infty < p < 1/2,
\end{align}
where the absolute approximate error is bounded by $0.005, \forall p \in [0.0075, 0.9925]$. In practice, we sample $m$ perturbations $\epsilon_1,\dots,\epsilon_m$ for each sample $x_i$, and optimize the importance sampled radius as
\begin{align}
    & \max_{\sigma > 0} R(\sigma, \theta, x_i, y_i, \epsilon) := \max_{\sigma > 0} \sigma \hat{\Phi}^{-1}(\frac{\bar{\sigma}^D}{\sigma^D} \sum_{j \in [m]}\bigg[ \frac
    {\prod_{k \in [D]}  \exp(-\epsilon_{j, k}^2 / 2\sigma^2))}
    {\prod_{k \in [D]} \exp(-\epsilon_{j, k}^2 / 2\bar{\sigma}^2)) }  P_\theta(y_i | x_i + \epsilon_j) \bigg]  ) 
\end{align}
Note that $P_\theta(y_i | x_i + \epsilon_j)$ only has to be computed once, so only the perturbations $\epsilon_i$ would be the bottleneck in GPU memory. 


The optimization problem can be solved in various ways:
\begin{itemize}
    \item Gradient ascent: 
    \begin{align}
        & \sigma_0 = \hat{\sigma} \\
        & \sigma_{t+1} = \sigma_t + \gamma_t \frac{\partial R(\sigma_t, \theta, x_i, y_i, \epsilon)}{\partial \sigma_t}
    \end{align}
    Cons: we have to tune the learning rate
    \item Newton's method. Cons: computation cost. 
    \item Fixed point equation: to satisfy the gradient optimality condition, the optimal $\sigma$ has the form
    \begin{align}
        & 0 = \frac{\partial R(\sigma_t, \theta, x_i, y_i, \epsilon)}{\partial \sigma_t} \\
        \iff & \sigma = \frac
        {- \hat{\Phi}^{-1}(\sum_{j \in [m]}\bigg[ \frac
    {\bar{\sigma}^D \prod_{k \in [D]}  \exp(-\epsilon_{j, k}^2 / 2\sigma^2))}
    {\sigma^D \prod_{k \in [D]} \exp(-\epsilon_{j, k}^2 / 2\bar{\sigma}^2)) }  P_\theta(y_i | x_i + \epsilon_j) \bigg]}
        {\frac{\partial}{\partial \sigma} \hat{\Phi}^{-1}(\sum_{j \in [m]}\bigg[ \frac
    {\bar{\sigma}^D \prod_{k \in [D]}  \exp(-\epsilon_{j, k}^2 / 2\sigma^2))}
    {\sigma^D \prod_{k \in [D]} \exp(-\epsilon_{j, k}^2 / 2\bar{\sigma}^2)) }  P_\theta(y_i | x_i + \epsilon_j) \bigg]}.
    \end{align}
    Pros: no need to tune the learning rate. Cons: it can also converge to the minimum. 
\end{itemize}
We denote the estimated $\sigma$ via the above procedure as $\hat{\sigma}(\theta, x_i, y_i, \epsilon)$.

\subsection{Optimize the model}

Note that the above derivation is based on a known label $y_i$, but it is infeasible in testing time to obtain the label, thus it is necessary to first predict the label $\hat{y}_i$ given $x_i$. To reflect this, we minimize the loss
\begin{align}
    \max\{0, \eta_1 + \max_{y \neq y_i} \sum_j P_\theta(y | x_i + \epsilon_j) - \sum_j P_\theta(y_i | x_i + \epsilon_j)\}
    %, \text{if } \sum_j P_\theta(y_i | x_i + \epsilon_j) > \max_{y \neq y_i} \sum_j P_\theta(y | x_i + \epsilon_j) + \eta_1.
\end{align}
where we may set $\eta_1 = 0.05$.

If the prediction is correct under the initial $\bar{\sigma}$ (the hinge is reached), we can then optimize the certificate $R$ explicitly as
\begin{align}
    & \max\{0, \eta_1 + \max_{y \neq y_i} \sum_j P_\theta(y | x_i + \epsilon_j) - \sum_j P_\theta(y_i | x_i + \epsilon_j)\} \\
    & + \max\{0, \alpha(\eta_2 - R(\sigma(\theta, x_i, y_i, \epsilon), \theta, x_i, y_i, \epsilon))\}.
\end{align}
where we may set $\eta_2 = \delta + 0.005 + \Delta, \alpha = 1/\Delta$. If $\delta \in \{1, 2, 4, 8\}$, we may set $\Delta = 0.1$

In testing time, we can simply first use the initial $\epsilon$ drawn from $\hat{\sigma}$, and then optimize $\sigma$ in the importance sampling form. Finally, we use the optimized $\sigma$ to find the certificate. 

\section{Problem Statement}

\begin{thm}
(CMU) Let $f: \mathbb{R}^d \to \mathcal{Y}$ be any deterministic or random function, and let $\epsilon \sim N(0, \sigma^2 I)$. Let 
\begin{align}
    & g(x) := \argmax_{c \in \mathcal{Y}} \mathbb{P}(f(x + \epsilon) = c)
\end{align}
Suppose $\underline{p_A}, \overline{P} \in [0, 1]$ are such that:
\begin{equation}
    \mathbb{P}(f(x+\epsilon) = c_A) \geq \underline{p_A} \geq \overline{P} \geq \max_{c \neq c_A} \mathbb{P}(f(x+\epsilon) = c)
\end{equation}
Then $g(x) = g(x + \delta)$ whenever $\|\delta\|_2 < R$, where
\begin{equation}
    R := \frac{\sigma}{2} (\Phi^{-1}(\underline{p_A}) - \Phi^{-1}(\overline{P})).
\end{equation}
\end{thm}

\begin{prop}
(CMU - 2) Let $f: \mathbb{R}^d \to \mathcal{Y}$ be any deterministic or random function, and let $\epsilon \sim N(0, \sigma^2 I)$. Let 
\begin{align}
    & g(x) := \argmax_{c \in \mathcal{Y}} \mathbb{P}(f(x + \epsilon) = c)
\end{align}
Suppose $\underline{p_A} > 0.5$ are such that:
\begin{equation}
    \mathbb{P}(f(x+\epsilon) = c_A) \geq \underline{p_A} \geq (1 - \underline{p_A}) \geq \max_{c \neq c_A} \mathbb{P}(f(x+\epsilon) = c)
\end{equation}
Then $g(x) = g(x + \delta)$ whenever $\|\delta\|_2 < R$, where
\begin{equation}
    R := \frac{\sigma}{2} (\Phi^{-1}(\underline{p_A}) - \Phi^{-1}(1 - \underline{p_A})) = \sigma \Phi^{-1}(\underline{p_A}).
\end{equation}
\end{prop}
We may assume $\epsilon = \|\delta\|_2$ is a fixed, given radius that we want to enforce robustness, and $\sigma$ is a hyper-parameter. The loss at testing time is thus:
\begin{equation}
    \frac{1}{n} \sum_{i \in [n]} \mathbb{I} (\sigma \Phi^{-1}(\mathbb{P}(f(x_i + \epsilon) = y_i) ) > \epsilon)
\end{equation}
Our first attempt is to rewrite the above objective as
\begin{equation}
    \frac{1}{n} \sum_{i \in [n]} \mathbb{I} (\mathbb{P}(f(x_i + \epsilon) = y_i) > \Phi(\frac{\epsilon}{\sigma}) ) = \frac{1}{n} \sum_{i \in [n]} \mathbb{I} (\mathbb{P}(f(x_i + \epsilon) = y_i) > \eta) ), \eta := \Phi(\frac{\epsilon}{\sigma}) \in [0, 1].
\end{equation}
Then we formulate an convex upper-bound of the loss for training. We may let $\beta = 0.5 (1 - \eta)$ and $\alpha = \frac{2}{1 - \eta}$, and we have:
\begin{equation}
    \frac{1}{n} \sum_{i \in [n]} \max \{0, \alpha ( \eta - \mathbb{P}(f(x_i + \epsilon) = y_i) + \beta ) \}.
\end{equation}
We also assume $f(x)$ is a randomized function, where each coordinate $f(x)_c$ encodes the probability to output class $c$, then we have:
\begin{equation}
    \mathbb{P}(f(x_i + \epsilon) = y_i) = \mathbb{E}_{\epsilon}[f(x_i + \epsilon)_{y_i}]
\end{equation}
Finally, we write our loss function as:
\begin{equation}
    \frac{1}{n} \sum_{i \in [n]} \max \{0, \alpha ( \eta - \mathbb{E}_{\epsilon}[f(x_i + \epsilon)_{y_i}] + \beta ) \}.
\end{equation}
To optimize $f$, for each $x_i$, we draw $m$ samples from the Gaussian distribution $\epsilon_1,\dots,\epsilon_m$. If 
\begin{equation}
   0 > \alpha ( \eta - \frac{1}{m} \sum_{j \in [m]} [f(x_i + \epsilon_j)_{y_i}] + \beta ),
\end{equation}
then the gradient w.r.t. $f$ is estimated to be $0$. Otherwise, the gradient w.r.t. $f$ is estimated by:
\begin{equation}
   \nabla \alpha ( \eta - \frac{1}{m} \sum_{j \in [m]} [f(x_i + \epsilon_j)_{y_i}] + \beta ),
\end{equation}


\section{Sampling method has bias}

We first show that to find a good solution, one should not train the model based on the noisy version of the dataset. 

\begin{lem}
For training set $Z=\{(x_1,y_1), \cdots, (x_n,y_n)\}$, if we consider the noisy version $Z'=\{(s_i^j,y_i)\}$ for $i\in[n], j\in [m]$, where $s_i^j=x_i+\xi_i^j$, $\xi_i^j\sim \N(\zero,\I)$. If we directly optimize our model using $Z'$, there may exists a constant gap between the final loss and the optimal adversarial loss.
\end{lem}
\begin{proof}
It suffices to prove this lemma by showing a bad example. 

Think about the following scenario. We have two classes, $+1$, and $-1$, and we consider the case where the adversarial perturbation is $\eps$. Consider one dimensional data $x\in \R$, where $x=-\eps/2$ or $\eps/2$ with equal probability and $y=\sign(x)$. In this example, we are learning threshold functions, defined as  $f_{a,b} (x)=  b\cdot \sign (x-a)$ for $a\in \R, b\in {\pm 1}$. We use $0$-$1$ loss. 

Now think about the case where $n=2$, $x_1=\eps/2$, $x_2=-\eps/2$. 
Assume that we pick $m$ sampled points around each input $x_i$ for really large $m$. If we directly optimize our model using $Z'$, we are dealing with $2m$ data points, and try to minimize the following loss function:
\[
\frac 1 {2m} \sum_{i=1}^{2m} \ell (f(s_i^j), y_i)
\]

Notice that $s_i^j$ is the noisy version of $x_i$, where the noise comes from Gaussian distribution. Therefore, by symmetry, we know that there will be more points with $-1$ labels for $s_i^j<0$, and more points with $+1$ labels for $s_i^j\geq 0$. (This can be shown using simple concentration, which we omit here)

That means, to minimize the loss function, we should pick $a=0, b=1$. 
However, simple calculation shows that this will give us $0$ accuracy under $\eps$ perturbation on the original input dataset $X$. 
A better solution is setting $a=\eps, b=1$. By doing this, we will get $50\%$ accuracy. 
\end{proof}

Instead of optimizing the noisy dataset, we can optimize the aggregate dataset, which is defined as follows. For every pair $(x_i, y_i)$, we define its aggregate dataset as $\{(s_i^j,y_i)\}$ for $j\in [m]$. Given a model $f$, define $P_A=\frac1m \sum_{j\in [m]} \one(f(s_i^j)=y_i)$ as the probability that our function gets the correct label, and $P=1-P_A$ which denotes the probability that our function gets the wrong label. We want to have that $P_A-P_B> \delta$ for some fixed $\delta>0$ to ensure robustness again $\eps$ perturbation. 

More specifically, we use the following loss function:
\[
L(f,x_i,y_i)=\max(0, P_A-\delta+1)
\]

If we use this loss for the example that we discussed above, it is clear that we will find the optimal loss, rather than get stuck at $a=0, b=1$. 

However, one problem of this approach is the gradient is biased after the aggregation step, when passing into the non-linear loss function. Fortunately,  (Chen \& Luss 2018) shows as long as the gradient estimate is consistent, SGD will still converge. Consistency is defined as follows. 

\begin{definition}
An estimator $g^N$ of $h$, where $N$ denotes the sample size, is consistent if $g^N$ converges to $h$ in probability: 
$\mathrm{plim}_{N\rightarrow \infty}  g^N=h$. That is, for any $\eps>0$, 
\[
\lim_{N\rightarrow \infty } \Pr(\|g^N-h\|>\eps)=0
\]
\end{definition}

For consistent estimators $g^N$, we use the following assumption to ensure the distance between $g^N$ and $h$ is not far away: 

\begin{assump}
There exists sample size $N_1, \cdots, N_T$ such that for every $i\in [T]$, we have
\[
\Pr(\|g_i^{N_i}-h_i\|\geq \delta \|h_i\|)\leq \eps
\]
\end{assump}
In other words, we know that we can pick finite number of samples such that in every step, our estimator is close to its expectation. 

We also need the following norm  upper bound on the estimator, which is standard for SGD analysis. 

\begin{assump}
There exists a finite $G>0$ such that $\|h\|\leq G$ for all gradient $h$.
\end{assump}

With these assumptions, (Chen \& Luss 2018) showed the following theorem.
\begin{lem}
If $f$ is $l$-strongly convex. For $T>3$ steps, with diminishing step size:
\[
\gamma_k =\frac1{(l-\delta)k}, k=1, 2, \cdots, T
\]
where $\delta=p/T$, and $p<l$ is an arbitrary constant indepdent of $T$. Then for any such $p$, and $\eps\in (0,1)$, and sufficiently large sample sizes, with probability at least $1-\eps$, we have 
\[
\|w_T-w^*\|_2\leq O(\frac{G^2}{T})
\]
and 
\[
f(\bar w_T) -f(w^*) \leq O(\frac{G^2}{T})
\]
where $\bar w_T\triangleq \frac{\sum_{i=1}^T w_i}{T}$
\end{lem}

One can show similar claims are true for general convex functions. For non-convex function, one gets $O(1/\sqrt{T})$ rate for the norm of the gradients. That is, converging to a stationary point. 

==> prelim.tex <==
%-------------------------------------------------------------------------


% we denote the set of measurable classifiers with respect to the perturbation $\rand$ as $\gF$, and consider the randomly smoothed classifier $f(\rand(\vx)) \in \gF$ for an $f \in \gF$, where the probability for outputting a class $c \in \gC$ is denoted as $\Pr(f(\phi(\vx))=c)$. 
% Note that $f$ can also be a random function. 
% Under this setting, we first develop tight robustness guarantees of the probability $\Pr(f(\phi(\vx))=c)$ with applications to robustness in accuracy and area under the ROC curve (AUC) in \xref{sec:certificates}, exemplify the framework in \xref{sec:examples}, and illustrate how the guarantees can be refined with further assumption in \xref{sec:refinement}. 

% In this work, we consider measurable classifiers $f$ with respect to a given perturbation, and use the probability that the randomly smoothed classifier outputs a class $c \in \gC$, $\Pr(f(\phi(\vx))=c)$, as the prediction probability

% develop robustness guarantees of the probability value of the compositie
% \begin{align}
%     \sE [ \one(f(\phi(\vx))=c) ] = \Pr(f(\phi(\vx))=c),
% \end{align}
% where $c \in \gC$ is a label 

% a measurable classifier $f$ with inputs randomly perturbed by a distribution $\phi$. 

% classifier $f: \gX \to \gC$ randomly smoothed by a perturbation function $\phi$, associated with a probability mass/density $\Pr(\rand(\vx) = \vz)$ for each perturbed outcome $\vz \in \gX$. The smoothed classifier is a co

% the class of ``randomly smoothed'' classifiers, which is defined as the compositions of a random perturbation function $\phi: \gX \to \gX$, which assigns , and a classifier $f: \gX \to \gC$. 

% In this paper, we consider the class of randomly smoothed classifiers, defining as 

% We assume that the input data lie in the domain $\gX \subseteq \sR^D$, the output data lie in the target set $\gC$.
% In this paper, we adopt a random perturbation function $\rand$ to input  $\vx\in \gX$, which assigns a probability mass/density $\Pr(\rand(\vx) = \vz)$ for each perturbed outcome $\vz \in \gX$. 
% A simple example would be 
% % $\gX = \sR^d$, and 
% $\rand(\vx) = \vx+ \veps$ with $\veps \sim \gN(0, I)$~\cite{cohen2019certified}.
% % , but more general random transformations can also be used, as we will see later. 
% Therefore, $f(\rand(\vx))$ represents a probability distribution over $\gC$, rather than a deterministic value. 

% We denote the set of all possible measurable functions $\tilde \gF_{\gX, \gC}\triangleq \{f: f\in \gX\rightarrow \gC\}$, and the set of candidate functions for our task $\gF_{\gX, \gC}\subseteq \tilde \gF_{\gX, \gC}$. When $\gX, \gC$ are clearly defined, we drop the subscripts for $\gF_{\gX, \gC}$ and $\tilde \gF_{\gX, \gC}$ for notational simplicity.
% We denote the $\ell_q$-norm ball with radius $r$ around $\vx$ as $\gB_{r, q}(\vx) \triangleq \{\bar \vx \in \gX: \|\bar \vx - \vx\|_q \leq r\}$.


% Given two points $\vx, \bar \vx \in \gX$, for any point $\vz \in \gX$, denote the likelihood ratio $\eta_{\vx, \bar \vx}(\vz)\triangleq \Pr(\rand(\vx) = \vz)/\Pr(\rand(\bar \vx) = \vz)$. 
% To simplify the notation, 
% below we drop the subscripts of $\eta$ as $\vx, \bar \vx$ are always clearly defined. If $\gX$ is discrete, 
% we can split it into $n$ disjoint regions $\gL_1,\dots,\gL_n: \cup_{i=1}^n \gL_i = \gX$ such that the likelihood ratio within each region is a constant $\eta_i$: $\forall i \in [n], \vz \in \gL_i, \eta(\vz) = \eta_i$. 
% In this case, we can sort the regions by the likelihood ratio such that $\eta_1 \geq \eta_2 \geq \dots \geq \eta_n\geq 0$.

% In binary classification,  we usually compute a score $s(x)$ for each input $x\in \gX$. We can denote $X_1$ ($X_0$) as a random variable to represent  the score of positive (negative) instances sampled from the data distribution.
% Given a threshold parameter $t$, we can classify $x$ as positive if $s(X)>t$, and vice versa. We define $\mathrm{TPR}(t)\triangleq \Pr(X_1\geq t)$, and $\mathrm{FPR}(t)\triangleq \Pr(X_0\geq t)$.

% A receiver operating characteristic (ROC) curve is a graphical plot for illustrating the performance of 
% a binary classification method with various thresholds. ROC curve is particularly useful when the two classes are imbalanced, which means the classification accuracy can be easily fooled. One popular interpretation of the ROC curve is called area under the curve (AUC). Mathematically, AUC is defined as:
% \begin{equation}
% \mathrm{AUC}=\int_{t=0}^1 \mathrm{TPR}(\mathrm{FPR}^{-1}(t)) \mathrm{dt}=P(X_1>X_0)
% \label{def:auc}
% \end{equation}



%-------------------------------------------------------------------------


==> tightness.tex <==

%\section{Tightness}







%\subsection{Exploiting structures of the model}
%
%If we know that the model only makes use the $d' < d$ dimensions, we can simply solve the minimization problem in Eq.~(\ref{eq:main_lemma}) by considering a smaller functional set $\gF' \subset \gF$ that only makes use of $d'$ dimensions to obtain a tighter bound by Remark~\ref{rmk:tight}.
%If $\gF = \tilde \gF$, we can equivalently cast the problem as minimizing over $\tilde \gF$ but in a lower dimensional space $\sR^{d'}$, and we can solve the minimax problem in the original framework. 
%
%
%We know for an input $\vx$, the output of a soft decision has the following form:
%
%\begin{align}
%\sum_{i=1}^L \prod_{k=1}^{N_i} \alpha^{\one\{\vx_{d(i, j)} \geq 0.5\}} \beta^{\one\{\vx_{d(i, j)} < 0.5\}},
%\end{align}
%for some $d: [L] \times [\text{max depth}] \to [D]$ and $\tau: [L] \times [\text{max depth}] \to $

% \subsection{Adding additional cues}
% Lemma~\ref{lem:clean_general} is tight with respect to a single point $\vx$. However, when we have the total control of the mapping $f$, we may compute the probability $\Pr(f(\rand(\vx'))=c), \forall \vx' \in \gX$ to further tighten the bound. For simplicity, we do so by only adding a point $\vx'$ with prediction probability $p'$ in the minimization problem:
% \begin{align}
%     \min_{\bar f \in \gF, \bar{\vx} \in \gB_{r, q}(\vx)} & \Pr(\bar{f}(\rand(\bar{\vx})) = c),\;\; s.t. \Pr(\bar f (\rand (\vx) = c)) = p, \Pr(\bar f (\rand (\vx')) = c) = p'.
% \end{align}
% This problem is more challenging to solve, though. Here we consider a simple case when $\gF = \tilde \gF$, and our discrete perturbation. For each $r \in \sZ_{\geq0}$, we know the following:
% \begin{align}
%     \|\vx - \bar \vx\|_0 = r, \|\vx - \vx'\|_0 = r',
% \end{align}
% which implies
% \begin{align}
%     |r - r'| \leq \|\vx' - \bar \vx\|_0 \leq r + r'
% \end{align}
% by triangle inequality. Hence, there are only $r + r' - |r - r'| + 1$ possible distances between $\vx'$ and $\bar \vx$. We may re-write
% \begin{align}
%     \min_{|r - r'| \leq r'' \leq r + r'} & \min_{\bar f \in \gF, \bar{\vx} \in \gB_{r, q}(\vx) \cap \gB_{r'', q}(\vx')} \Pr(\bar{f}(\rand(\bar{\vx})) = c)\\
%     s.t.& \Pr(\bar f (\rand (\vx) = c)) = p, \Pr(\bar f (\rand (\vx')) = c) = p'.
% \end{align}
% Then for each $r''$, there are at most $(d+1)^3$ possible regions with different likelihood with respect to $\vx, \vx'$ and $\bar \vx$, respectively. By a similar argument to Theorem 1, we may solve the program for each $r''$ as
% \begin{align}
%     \min_{\bar f \in \gF, \bar{\vx} \in \gB_{r, q}(\vx) \cap \gB_{r'', q}(\vx')} & \Pr(\bar{f}(\rand(\bar{\vx})) = c)\\
%     s.t.& \Pr(\bar f (\rand (\vx) = c)) = p, \Pr(\bar f (\rand (\vx')) = c) = p'. \\
%     = \min_{\one^*: [(d+1)^3] \to [0, 1]} & \sum_{i=1}^{(d+1)^3} \Pr(\rand(\bar \vx) \in \gL_i) \one^*(i) \\
%     s.t.& \sum_{i=1}^{(d+1)^3} \Pr(\rand(\vx) \in \gL_i)  \one^*(i) = p \\
%         & \sum_{i=1}^{(d+1)^3} \Pr(\rand(\vx') \in \gL_i) \one^*(i) = p', \\
% \end{align}
% which is a linear program. \textred{Need proof? Seems straightforward...}
